Defenses in Adversarial Machine Learning: A Survey

Adversarial phenomenon has been widely observed in machine learning (ML) systems, especially in those using deep neural networks, describing that ML systems may produce inconsistent and incomprehensible predictions with humans at some particular cases. This phenomenon poses a serious security threat to the practical application of ML systems, and several advanced attack paradigms have been developed to explore it, mainly including backdoor attacks, weight attacks, and adversarial examples. For each individual attack paradigm, various defense paradigms have been developed to improve the model robustness against the corresponding attack paradigm. However, due to the independence and diversity of these defense paradigms, it is difficult to examine the overall robustness of an ML system against different kinds of attacks.This survey aims to build a systematic review of all existing defense paradigms from a unified perspective. Specifically, from the life-cycle perspective, we factorize a complete machine learning system into five stages, including pre-training, training, post-training, deployment, and inference stages, respectively. Then, we present a clear taxonomy to categorize and review representative defense methods at each individual stage. The unified perspective and presented taxonomies not only facilitate the analysis of the mechanism of each defense paradigm but also help us to understand connections and differences among different defense paradigms, which may inspire future research to develop more advanced, comprehensive defenses.

==> backup_reference.tex <==
%-------------------------
% related survey 
%-------------------------

@article{wu2023adversarial,
  title={Adversarial machine learning: A systematic survey of backdoor attack, weight attack and adversarial example},
  author={Wu, Baoyuan and Liu, Li and Zhu, Zihao and Liu, Qingshan and He, Zhaofeng and Lyu, Siwei},
  journal={arXiv preprint arXiv:2302.09457},
  year={2023}
}

@article{wei2022physically,
  title={Physically adversarial attacks and defenses in computer vision: a survey},
  author={Wei, Xingxing and Pu, Bangzheng and Lu, Jiefan and Wu, Baoyuan},
  journal={arXiv preprint arXiv:2211.01671},
  year={2022}
}

@article{gao2020backdoor,
  title={Backdoor attacks and countermeasures on deep learning: A comprehensive review},
  author={Gao, Yansong and Doan, Bao Gia and Zhang, Zhi and Ma, Siqi and Zhang, Jiliang and Fu, Anmin and Nepal, Surya and Kim, Hyoungshick},
  journal={arXiv preprint arXiv:2007.10760},
  year={2020}
}

@article{goldblum2022dataset,
  title={Dataset security for machine learning: Data poisoning, backdoor attacks, and defenses},
  author={Goldblum, Micah and Tsipras, Dimitris and Xie, Chulin and Chen, Xinyun and Schwarzschild, Avi and Song, Dawn and M{\k{a}}dry, Aleksander and Li, Bo and Goldstein, Tom},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={2},
  pages={1563--1580},
  year={2022},
  publisher={IEEE}
}

@article{qian2022survey,
  title={A survey of robust adversarial training in pattern recognition: Fundamental, theory, and methodologies},
  author={Qian, Zhuang and Huang, Kaizhu and Wang, Qiu-Feng and Zhang, Xu-Yao},
  journal={Pattern Recognition},
  volume={131},
  pages={108889},
  year={2022},
  publisher={Elsevier}
}

@article{qian2023survey,
  title={A Survey of bit-flip attacks on deep neural network and corresponding defense methods},
  author={Qian, Cheng and Zhang, Ming and Nie, Yuanping and Lu, Shuaibing and Cao, Huayang},
  journal={Electronics},
  volume={12},
  number={4},
  pages={853},
  year={2023},
  publisher={MDPI}
}


%-------------------------
% pre-training stage defense 
%-------------------------

% robust model architecture
@inproceedings{jung2023neural,
  title={Neural Architecture Design and Robustness: A Dataset},
  author={Jung, Steffen and Lukasik, Jovita and Keuper, Margret},
  booktitle={Eleventh International Conference on Learning Representations},
  year={2023}
}

@article{huang2021exploring,
  title={Exploring architectural ingredients of adversarially robust deep neural networks},
  author={Huang, Hanxun and Wang, Yisen and Erfani, Sarah and Gu, Quanquan and Bailey, James and Ma, Xingjun},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={5545--5559},
  year={2021}
}

@article{peng2023robarch,
  title={RobArch: Designing Robust Architectures against Adversarial Attacks},
  author={Peng, ShengYun and Xu, Weilin and Cornelius, Cory and Li, Kevin and Duggal, Rahul and Chau, Duen Horng and Martin, Jason},
  journal={arXiv preprint arXiv:2301.03110},
  year={2023}
}

@article{wu2021wider,
  title={Do wider neural networks really help adversarial robustness?},
  author={Wu, Boxi and Chen, Jinghui and Cai, Deng and He, Xiaofei and Gu, Quanquan},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={7054--7067},
  year={2021}
}

@inproceedings{guo2020meets,
  title={When nas meets robustness: In search of robust architectures against adversarial attacks},
  author={Guo, Minghao and Yang, Yuzhe and Xu, Rui and Liu, Ziwei and Lin, Dahua},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={631--640},
  year={2020}
}

@inproceedings{hosseini2021dsrna,
  title={Dsrna: Differentiable search of robust neural architectures},
  author={Hosseini, Ramtin and Yang, Xingyi and Xie, Pengtao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={6196--6205},
  year={2021}
}

@inproceedings{chen2020anti,
  title={Anti-bandit neural architecture search for model defense},
  author={Chen, Hanlin and Zhang, Baochang and Xue, Song and Gong, Xuan and Liu, Hong and Ji, Rongrong and Doermann, David},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XIII 16},
  pages={70--85},
  year={2020},
  organization={Springer}
}


@inproceedings{bu2023towards,
  title={Towards Building More Robust Models with Frequency Bias},
  author={Bu, Qingwen and Huang, Dong and Cui, Heming},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={4402--4411},
  year={2023}
}

@article{Tang2023SettingTT,
  title={Setting the Trap: Capturing and Defeating Backdoors in Pretrained Language Models through Honeypots},
  author={Ruixiang Tang and Jiayi Yuan and Yiming Li and Zirui Liu and Rui Chen and Xia Hu},
  journal={ArXiv},
  year={2023},
  volume={abs/2310.18633},
  url={https://api.semanticscholar.org/CorpusID:264590464}
}


% data pre-processing based defense
@inproceedings{asset,
  author       = {Minzhou Pan and
                  Yi Zeng and
                  Lingjuan Lyu and
                  Xue Lin and
                  Ruoxi Jia},
  title        = {{ASSET:} Robust Backdoor Data Detection Across a Multiplicity of Deep Learning Paradigms},
  booktitle    = {32nd {USENIX} Security Symposium, {USENIX} Security 2023},
  publisher    = {{USENIX} Association},
  year         = {2023}
}
@inproceedings{du2020robust,
  title={Robust anomaly detection and backdoor attack detection via differential privacy},
  author={Du, Min and Jia, Ruoxi and Song, Dawn},
  booktitle={International Conference on Learning Representations},
  year={2020}
}
@inproceedings {demon,
author = {Di Tang and XiaoFeng Wang and Haixu Tang and Kehuan Zhang},
title = {Demon in the Variant: Statistical Analysis of {DNNs} for Robust Backdoor Contamination Detection},
booktitle = {30th USENIX Security Symposium (USENIX Security 21)},
year = {2021},
pages = {1541--1558},
publisher = {USENIX Association}
}

@inproceedings{al2023don,
  title={Don't FREAK Out: A Frequency-Inspired Approach to Detecting Backdoor Poisoned Samples in DNNs},
  author={Al Kader Hammoud, Hasan Abed and Bibi, Adel and Torr, Philip HS and Ghanem, Bernard},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2337--2344},
  year={2023}
}

@inproceedings{hammoudeh2022identifying,
  title={Identifying a training-set attack's target using renormalized influence estimation},
  author={Hammoudeh, Zayd and Lowd, Daniel},
  booktitle={Proceedings of the 2022 ACM SIGSAC Conference on Computer and Communications Security},
  pages={1367--1381},
  year={2022}
}

@inproceedings{du2019robust,
  title={Robust anomaly detection and backdoor attack detection via differential privacy},
  author={Du, Min and Jia, Ruoxi and Song, Dawn},
  booktitle={International Conference on Learning Representations},
  year={2019}
}

@inproceedings{chou2020sentinet,
  title={Sentinet: Detecting localized universal attacks against deep learning systems},
  author={Chou, Edward and Tramer, Florian and Pellegrino, Giancarlo},
  booktitle={2020 IEEE Security and Privacy Workshops (SPW)},
  pages={48--54},
  year={2020},
  organization={IEEE}
}

@inproceedings{hayase2021spectre,
  title={Spectre: Defending against backdoor attacks using robust statistics},
  author={Hayase, Jonathan and Kong, Weihao and Somani, Raghav and Oh, Sewoong},
  booktitle={International Conference on Machine Learning},
  pages={4129--4139},
  year={2021},
  organization={PMLR}
}

@inproceedings{gao2019strip,
  title={Strip: A defence against trojan attacks on deep neural networks},
  author={Gao, Yansong and Xu, Change and Wang, Derui and Chen, Shiping and Ranasinghe, Damith C and Nepal, Surya},
  booktitle={Proceedings of the 35th Annual Computer Security Applications Conference},
  pages={113--125},
  year={2019}
}

@inproceedings{beatrix,
  author       = {Wanlun Ma and Derui Wang and Ruoxi Sun and Minhui Xue and Sheng Wen and Yang Xiang},
  title        = {The "Beatrix" Resurrections: Robust Backdoor Detection via Gram Matrices},
  booktitle    = {30th Annual Network and Distributed System Security Symposium},
  publisher    = {The Internet Society},
  year         = {2023}
}

@inproceedings{qitowards,
  title={Towards A Proactive ML Approach for Detecting Backdoor Poison Samples},
  author={Qi, Xiangyu and Xie, Tinghao and Wang, Tianhao and Wu, Tong and Mahloujifar, Saeed and Mittal, Prateek},
  booktitle={USENIX Security Symposium},
  year={2023}
}

%-------------------------
% training stage defense 
%-------------------------

%---------- training-stage defense against adversarial attack
@inproceedings{bui2022unified,
title = {A Unified Wasserstein Distributional Robustness Framework for Adversarial Training},
author = {Anh Tuan Bui and Trung Le and Quan Hung Tran and He Zhao and Dinh Q. Phung},
booktitle = {ICLR 2022},
year = {2022}
}

@inproceedings{dong2020adversarial,
title = {Adversarial Distributional Training for Robust Deep Learning},
author = {Yinpeng Dong and Zhijie Deng and Tianyu Pang and Jun Zhu and Hang Su},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{maini2020adversarial,
title = {Adversarial Robustness Against the Union of Multiple Perturbation Models},
author = {Pratyush Maini and Eric Wong and J. Zico Kolter},
booktitle = {ICML 2020},
volume = {119},
pages = {6640--6650},
year = {2020}
}

@inproceedings{fan2021adversarial,
title = {Adversarial Training and Provable Robustness: {A} Tale of Two Objectives},
author = {Jiameng Fan and Wenchao Li},
booktitle = {AAAI 2021},
pages = {7367--7376},
year = {2021}
}

@inproceedings{tramer2019adversarial,
title = {Adversarial Training and Robustness for Multiple Perturbations},
author = {Florian Tram{\`{e}}r and Dan Boneh},
booktitle = {NeurIPS 2019},
pages = {5858--5868},
year = {2019}
}

@inproceedings{shafahi2019adversarial,
title = {Adversarial training for free!},
author = {Ali Shafahi and Mahyar Najibi and Amin Ghiasi and Zheng Xu and John P. Dickerson and Christoph Studer and Larry S. Davis and Gavin Taylor and Tom Goldstein},
booktitle = {NeurIPS 2019},
pages = {3353--3364},
year = {2019}
}



@inproceedings{roth2020adversarial,
title = {Adversarial Training is a Form of Data-dependent Operator Norm Regularization},
author = {Kevin Roth and Yannic Kilcher and Thomas Hofmann},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{mendoncca2022adversarial,
title = {Adversarial training with informed data selection},
author = {Mendon{\c{c}}a, Marcele OK and Maroto, Javier and Frossard, Pascal and Diniz, Paulo SR},
booktitle = {EUSIPCO 2022},
pages = {608--612},
organization = {IEEE},
year = {2022}
}

@inproceedings{lee2020adversarial,
title = {Adversarial Vertex Mixup: Toward Better Adversarially Robust Generalization},
author = {Saehyung Lee and Hyungyu Lee and Sungroh Yoon},
booktitle = {CVPR 2020},
pages = {269--278},
year = {2020}
}

@inproceedings{wu2020adversarial,
title = {Adversarial Weight Perturbation Helps Robust Generalization},
author = {Dongxian Wu and Shu{-}Tao Xia and Yisen Wang},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{wallace2021analyzing,
title = {Analyzing Dynamic Adversarial Training Data in the Limit},
author = {Wallace, Eric  and Williams, Adina  and Jia, Robin  and Kiela, Douwe},
booktitle = {ACL 2022},
pages = {202--217},
year = {2022}
}

@inproceedings{alayrac2019labels,
title = {Are Labels Required for Improving Adversarial Robustness?},
author = {Jean{-}Baptiste Alayrac and Jonathan Uesato and Po{-}Sen Huang and Alhussein Fawzi and Robert Stanforth and Pushmeet Kohli},
booktitle = {NeurIPS 2019},
pages = {12192--12202},
year = {2019}
}

@inproceedings{zhang2020attacks,
title = {Attacks Which Do Not Kill Training Make Adversarial Learning Stronger},
author = {Jingfeng Zhang and Xilie Xu and Bo Han and Gang Niu and Lizhen Cui and Masashi Sugiyama and Mohan S. Kankanhalli},
booktitle = {ICML 2020},
volume = {119},
pages = {11278--11287},
year = {2020}
}

@inproceedings{wang2019bilateral,
title = {Bilateral Adversarial Training: Towards Fast Training of More Robust Models Against Adversarial Attacks},
author = {Jianyu Wang and Haichao Zhang},
booktitle = {ICCV 2019},
pages = {6628--6637},
year = {2019}
}

@inproceedings{kanai2023one,
  title={One-vs-the-Rest Loss to Focus on Important Samples in Adversarial Training},
  author={Kanai, Sekitoshi and Yamaguchi, Shin’Ya and Yamada, Masanori and Takahashi, Hiroshi and Ohno, Kentaro and Ida, Yasutoshi},
  booktitle={International Conference on Machine Learning},
  pages={15669--15695},
  year={2023},
  organization={PMLR}
}

@article{yang2023improving,
  title={Improving Adversarial Robustness by Putting More Regularizations on Less Robust Samples},
  author={Yang, Dongyoon and Kong, Insung and Kim, Yongdai},
  year={2023}
}

@inproceedings{ghamizi2023gat,
  title={GAT: Guided Adversarial Training with Pareto-optimal Auxiliary Tasks},
  author={Ghamizi, Salah and Zhang, Jingfeng and Cordy, Maxime and Papadakis, Mike and Sugiyama, Masashi and Le Traon, Yves},
  booktitle={International Conference on Machine Learning},
  pages={11255--11282},
  year={2023},
  organization={PMLR}
}

@article{zhou2023phase,
  title={Phase-aware Adversarial Defense for Improving Adversarial Robustness},
  author={Zhou, Dawei and Wang, Nannan and Yang, Heng and Gao, Xinbo and Liu, Tongliang},
  year={2023}
}

@inproceedings{jiang2023towards,
  title={Towards Stable and Efficient Adversarial Training against $ l\_1 $ Bounded Adversarial Attacks},
  author={Jiang, Yulun and Liu, Chen and Huang, Zhichao and Salzmann, Mathieu and Susstrunk, Sabine},
  booktitle={International Conference on Machine Learning},
  pages={15089--15104},
  year={2023},
  organization={PMLR}
}

@article{ye2021annealing,
  title={An annealing mechanism for adversarial training acceleration},
  author={Ye, Nanyang and Li, Qianxiao and Zhou, Xiao-Yun and Zhu, Zhanxing},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2021},
  publisher={IEEE}
}


@article{jia2022boosting,
title = {Boosting fast adversarial training with learnable adversarial initialization},
author = {Jia, Xiaojun and Zhang, Yong and Wu, Baoyuan and Wang, Jue and Cao, Xiaochun},
journal = {IEEE Transactions on Image Processing},
volume = {31},
pages = {4417--4430},
year = {2022}
}

@inproceedings{huang2021calibrated,
title = {calibrated adversarial training},
author = {Huang, Tianjin and Menkovski, Vlado and Pei, Yulong and Pechenizkiy, Mykola},
booktitle = {ACML 2021},
pages = {626--641},
organization = {PMLR},
year = {2021}
}

@article{wei2023cfa,
title = {CFA: Class-wise Calibrated Fair Adversarial Training},
author = {Wei, Zeming and Wang, Yifei and Guo, Yiwen and Wang, Yisen},
journal = {ArXiv preprint},
volume = {abs/2303.14460},
year = {2023}
}

@inproceedings{cai2018curriculum,
title = {Curriculum Adversarial Training},
author = {Qi{-}Zhi Cai and Chang Liu and Dawn Song},
booktitle = {IJCAI 2018},
pages = {3740--3747},
year = {2018}
}

@inproceedings{li2023data,
title={Data augmentation alone can improve adversarial training},
author={Lin Li and Michael W. Spratling},
booktitle = {ICLR 2023},
year={2023},
}

@inproceedings{mummadi2019defending,
title = {Defending Against Universal Perturbations With Shared Adversarial Training},
author = {Chaithanya Kumar Mummadi and Thomas Brox and Jan Hendrik Metzen},
booktitle = {ICCV 2019},
pages = {4927--4936},
year = {2019}
}

@inproceedings{zhang2019defense,
title = {Defense Against Adversarial Attacks Using Feature Scattering-based Adversarial Training},
author = {Haichao Zhang and Jianyu Wang},
booktitle = {NeurIPS 2019},
pages = {1829--1839},
year = {2019}
}

@inproceedings{staib2017distributionally,
title = {Distributionally robust deep learning as a generalization of adversarial training},
author = {Staib, Matthew and Jegelka, Stefanie},
booktitle = {NIPS 2017},
volume = {3},
pages = {4},
year = {2017}
}

@inproceedings{yang2020dverge,
title = {{DVERGE:} Diversifying Vulnerabilities for Enhanced Robust Generation of Ensembles},
author = {Huanrui Yang and Jingyang Zhang and Hongliang Dong and Nathan Inkawhich and Andrew Gardner and Andrew Touchet and Wesley Wilkes and Heath Berry and Hai Li},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{zheng2020efficient,
title = {Efficient Adversarial Training With Transferable Adversarial Examples},
author = {Haizhong Zheng and Ziqi Zhang and Juncheng Gu and Honglak Lee and Atul Prakash},
booktitle = {CVPR 2020},
pages = {1178--1187},
year = {2020}
}

@article{addepalli2022efficient,
title = {Efficient and effective augmentation strategy for adversarial training},
author = {Addepalli, Sravanti and Jain, Samyak and others},
journal = {Advances in Neural Information Processing Systems},
volume = {35},
pages = {1488--1501},
year = {2022}
}

@inproceedings{jin2022enhancing,
title = {Enhancing Adversarial Training with Second-Order Statistics of Weights},
author = {Gaojie Jin and Xinping Yi and Wei Huang and Sven Schewe and Xiaowei Huang},
booktitle = {CVPR 2022},
pages = {15252--15262},
year = {2022}
}

@inproceedings{tramer2017ensemble,
title = {Ensemble Adversarial Training: Attacks and Defenses},
author = {Florian Tram{\`{e}}r and Alexey Kurakin and Nicolas Papernot and Ian J. Goodfellow and Dan Boneh and Patrick D. McDaniel},
booktitle = {ICLR 2018},
year = {2018}
}

@inproceedings{ntk-at,
title={Evolution of Neural Tangent Kernels under Benign and Adversarial Training}, 
author={Noel Loo and Ramin Hasani and Alexander Amini and Daniela Rus},
booktitle = {NeurIPS 2022},
year={2022},
}

@inproceedings{dong2021exploring,
title = {Exploring Memorization in Adversarial Training},
author = {Yinpeng Dong and Ke Xu and Xiao Yang and Tianyu Pang and Zhijie Deng and Hang Su and Jun Zhu},
booktitle = {ICLR 2022},
year = {2022}
}

@inproceedings{wong2020fast,
title = {Fast is better than free: Revisiting adversarial training},
author = {Eric Wong and Leslie Rice and J. Zico Kolter},
booktitle = {ICLR 2020},
year = {2020}
}

@inproceedings{farnia2018generalizable,
title = {Generalizable Adversarial Training via Spectral Normalization},
author = {Farzan Farnia and Jesse M. Zhang and David Tse},
booktitle = {ICLR 2019},
year = {2019}
}

@inproceedings{vivek2018gray,
title = {Gray-box adversarial training},
author = {Vivek, BS and Mopuri, Konda Reddy and Babu, R Venkatesh},
booktitle = {ECCV 2018},
pages = {203--218},
year = {2018}
}

@inproceedings{sriramanan2020guided,
title = {Guided Adversarial Attack for Evaluating and Enhancing Adversarial Defenses},
author = {Gaurang Sriramanan and Sravanti Addepalli and Arya Baburaj and Venkatesh Babu R.},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{wang2022imbalanced,
title = {Imbalanced adversarial training with reweighting},
author = {Wang, Wentao and Xu, Han and Liu, Xiaorui and Li, Yaxin and Thuraisingham, Bhavani and Tang, Jiliang},
booktitle = {ICDM 2022},
pages = {1209--1214},
organization = {IEEE},
year = {2022}
}

@inproceedings{wang2020improving,
title = {Improving Adversarial Robustness Requires Revisiting Misclassified Examples},
author = {Yisen Wang and Difan Zou and Jinfeng Yi and James Bailey and Xingjun Ma and Quanquan Gu},
booktitle = {ICLR 2020},
year = {2020}
}

@inproceedings{gowal2021improving,
title = {Improving Robustness using Generated Data},
author = {Sven Gowal and Sylvestre{-}Alvise Rebuffi and Olivia Wiles and Florian Stimberg and Dan Andrei Calian and Timothy A. Mann},
booktitle = {NeurIPS 2021},
pages = {4218--4233},
year = {2021}
}

@inproceedings{song2018improving,
title = {Improving the Generalization of Adversarial Training with Domain Adaptation},
author = {Chuanbiao Song and Kun He and Liwei Wang and John E. Hopcroft},
booktitle = {ICLR 2019},
year = {2019}
}

@article{xu2022infoat,
title = {InfoAT: Improving Adversarial Training Using the Information Bottleneck Principle},
author = {Xu, Mengting and Zhang, Tao and Li, Zhongnian and Zhang, Daoqiang},
journal = {IEEE Transactions on Neural Networks and Learning Systems},
year = {2022}
}

@inproceedings{xie2019intriguing,
title = {Intriguing Properties of Adversarial Training at Scale},
author = {Cihang Xie and Alan L. Yuille},
booktitle = {ICLR 2020},
year = {2020}
}

@article{he2023investigating,
title = {Investigating Catastrophic Overfitting in Fast Adversarial Training: A Self-fitting Perspective},
author = {He, Zhengbao and Li, Tao and Chen, Sizhe and Huang, Xiaolin},
journal = {ArXiv preprint},
volume = {abs/2302.11963},
year = {2023}
}

@article{dong2022label,
title = {Label Noise in Adversarial Training: A Novel Perspective to Study Robust Overfitting},
author = {Dong, Chengyu and Liu, Liyuan and Shang, Jingbo},
journal = {Advances in Neural Information Processing Systems},
volume = {35},
pages = {17556--17567},
year = {2022}
}

@article{zhou2022ladder,
title = {LADDER: Latent boundary-guided adversarial training},
author = {Zhou, Xiaowei and Tsang, Ivor W and Yin, Jie},
journal = {Machine Learning},
pages = {1--29},
year = {2022}
}

@inproceedings{jia2022adversarial,
title = {{LAS-AT:} Adversarial Training with Learnable Attack Strategy},
author = {Xiaojun Jia and Yong Zhang and Baoyuan Wu and Ke Ma and Jue Wang and Xiaochun Cao},
booktitle = {CVPR 2022},
pages = {13388--13398},
year = {2022}
}

@inproceedings{cui2021learnable,
title = {Learnable Boundary Guided Adversarial Training},
author = {Jiequan Cui and Shu Liu and Liwei Wang and Jiaya Jia},
booktitle = {ICCV 2021},
pages = {15701--15710},
year = {2021}
}

@article{li2023less,
title = {Less is More: Data Pruning for Faster Adversarial Training},
author = {Li, Yize and Zhao, Pu and Lin, Xue and Kailkhura, Bhavya and Goldh, Ryan},
journal = {ArXiv preprint},
volume = {abs/2302.12366},
year = {2023}
}

@inproceedings{singla2021low,
title = {Low Curvature Activations Reduce Overfitting in Adversarial Training},
author = {Vasu Singla and Sahil Singla and Soheil Feizi and David Jacobs},
booktitle = {ICCV 2021},
pages = {16403--16413},
year = {2021}
}

@article{de2022make,
title = {Make some noise: Reliable and efficient single-step adversarial training},
author = {de Jorge Aranda, Pau and Bibi, Adel and Volpi, Riccardo and Sanyal, Amartya and Torr, Philip and Rogez, Gr{\'e}gory and Dokania, Puneet},
journal = {Advances in Neural Information Processing Systems},
volume = {35},
pages = {12881--12893},
year = {2022}
}

@inproceedings{mao2019metric,
title = {Metric Learning for Adversarial Robustness},
author = {Chengzhi Mao and Ziyuan Zhong and Junfeng Yang and Carl Vondrick and Baishakhi Ray},
booktitle = {NeurIPS 2019},
pages = {478--489},
year = {2019}
}

@inproceedings{ding2018mma,
title = {{MMA} Training: Direct Input Space Margin Maximization through Adversarial Training},
author = {Gavin Weiguang Ding and Yash Sharma and Kry Yik Chau Lui and Ruitong Huang},
booktitle = {ICLR 2020},
year = {2020}
}

@article{liu2022mutual,
title = {Mutual Adversarial Training: Learning together is better than going alone},
author = {Liu, Jiang and Lau, Chun Pong and Souri, Hossein and Feizi, Soheil and Chellappa, Rama},
journal = {IEEE Transactions on Information Forensics and Security},
volume = {17},
pages = {2364--2377},
year = {2022}
}

@article{zhang2022noilin,
title = {Noilin: Improving adversarial training and correcting stereotype of noisy labels},
author = {Zhang, Jingfeng and Xu, Xilie and Han, Bo and Liu, Tongliang and Cui, Lizhen and Niu, Gang and Sugiyama, Masashi},
year = {2022}
}

@inproceedings{wang2021convergence,
title = {On the Convergence and Robustness of Adversarial Training},
author = {Yisen Wang and Xingjun Ma and James Bailey and Jinfeng Yi and Bowen Zhou and Quanquan Gu},
booktitle = {ICML 2019},
volume = {97},
pages = {6586--6595},
year = {2019}
}

@inproceedings{jia2022prior,
title = {Prior-Guided Adversarial Initialization for Fast Adversarial Training},
author = {Jia, Xiaojun and Zhang, Yong and Wei, Xingxing and Wu, Baoyuan and Ma, Ke and Wang, Jue and Cao, Xiaochun},
booktitle = {ECCV 2022},
pages = {567--584},
organization = {Springer},
year = {2022}
}

@inproceedings{liu2021probabilistic,
title = {Probabilistic Margins for Instance Reweighting in Adversarial Training},
author = {Qizhou Wang and Feng Liu and Bo Han and Tongliang Liu and Chen Gong and Gang Niu and Mingyuan Zhou and Masashi Sugiyama},
booktitle = {NeurIPS 2021},
pages = {23258--23269},
year = {2021}
}

@inproceedings{herrmann2022pyramid,
title = {Pyramid Adversarial Training Improves ViT Performance},
author = {Charles Herrmann and Kyle Sargent and Lu Jiang and Ramin Zabih and Huiwen Chang and Ce Liu and Dilip Krishnan and Deqing Sun},
booktitle = {CVPR 2022},
pages = {13409--13419},
year = {2022}
}

@article{jin2023randomized,
title = {Randomized Adversarial Training via Taylor Expansion},
author = {Jin, Gaojie and Yi, Xinping and Wu, Dengyu and Mu, Ronghui and Huang, Xiaowei},
journal = {ArXiv preprint},
volume = {abs/2303.10653},
year = {2023}
}

@inproceedings{osada2020regularization,
title = {Regularization with latent space virtual adversarial training},
author = {Osada, Genki and Ahsan, Budrul and Bora, Revoti Prasad and Nishide, Takashi},
booktitle = {ECCV 2020},
pages = {565--581},
organization = {Springer},
year = {2020}
}

@inproceedings{park2021reliably,
title = {Reliably fast adversarial training via latent adversarial perturbation},
author = {Geon Yeong Park and Sang Wan Lee},
booktitle = {ICCV 2021},
pages = {7738--7747},
year = {2021}
}

@inproceedings{wang2022removing,
title = {Removing Batch Normalization Boosts Adversarial Training},
author = {Haotao Wang and Aston Zhang and Shuai Zheng and Xingjian Shi and Mu Li and Zhangyang Wang},
booktitle = {ICML 2022},
volume = {162},
pages = {23433--23445},
year = {2022}
}

@inproceedings{zhang2022revisiting,
title = {Revisiting and Advancing Fast Adversarial Training Through The Lens of Bi-Level Optimization},
author = {Yihua Zhang and Guanhua Zhang and Prashant Khanduri and Mingyi Hong and Shiyu Chang and Sijia Liu},
booktitle = {ICML 2022},
volume = {162},
pages = {26693--26712},
year = {2022}
}

@inproceedings{dabouei2022revisiting,
title = {Revisiting Outer Optimization in Adversarial Training},
author = {Dabouei, Ali and Taherkhani, Fariborz and Soleymani, Sobhan and Nasrabadi, Nasser M},
booktitle = {ECCV 2022},
pages = {244--261},
organization = {Springer},
year = {2022}
}

@inproceedings{xie2021robust,
title = {Robust single-step adversarial training with regularizer},
author = {Xie, Lehui and Wang, Yaopeng and Yin, Jia-Li and Liu, Ximeng},
booktitle = {PRCV 2021},
pages = {29--41},
organization = {Springer},
year = {2021}
}

@inproceedings{ijcai2022p512,
title     = {Robust Weight Perturbation for Adversarial Training},
author    = {Yu, Chaojian and Han, Bo and Gong, Mingming and Shen, Li and Ge, Shiming and Bo, Du and Liu, Tongliang},
booktitle = {IJCAI 2022},
pages     = {3688--3694},
year      = {2022},
}

@inproceedings{pang2022robustness,
title = {Robustness and Accuracy Could Be Reconcilable by (Proper) Definition},
author = {Tianyu Pang and Min Lin and Xiao Yang and Jun Zhu and Shuicheng Yan},
booktitle = {ICML 2022},
volume = {162},
pages = {17258--17277},
year = {2022}
}

@inproceedings{addepalli2022scaling,
title = {Scaling adversarial training to large perturbation bounds},
author = {Addepalli, Sravanti and Jain, Samyak and Sriramanan, Gaurang and Venkatesh Babu, R},
booktitle = {ECCV 2022},
pages = {301--316},
organization = {Springer},
year = {2022}
}

@inproceedings{wang2022self,
title = {Self-ensemble Adversarial Training for Improved Robustness},
author = {Hongjun Wang and Yisen Wang},
booktitle = {ICLR 2022},
year = {2022}
}

@article{li2022semi,
title = {Semi-supervised robust training with generalized perturbed neighborhood},
author = {Li, Yiming and Wu, Baoyuan and Feng, Yan and Fan, Yanbo and Jiang, Yong and Li, Zhifeng and Xia, Shu-Tao},
journal = {Pattern Recognition},
volume = {124},
pages = {108472},
year = {2022}
}

@inproceedings{li2023squeeze,
title = {Squeeze Training for Adversarial Robustness},
author = {Li, Qizhang and Guo, Yiwen and Zuo, Wangmeng and Chen, Hao},
booktitle = {ICLR 2023},
year = {2023}
}

@inproceedings{li2022subspace,
title = {Subspace Adversarial Training},
author = {Tao Li and Yingwen Wu and Sizhe Chen and Kun Fang and Xiaolin Huang},
booktitle = {CVPR 2022},
pages = {13399--13408},
year = {2022}
}

@inproceedings{zhang2019theoretically,
title = {Theoretically Principled Trade-off between Robustness and Accuracy},
author = {Hongyang Zhang and Yaodong Yu and Jiantao Jiao and Eric P. Xing and Laurent El Ghaoui and Michael I. Jordan},
booktitle = {ICML 2019},
volume = {97},
pages = {7472--7482},
year = {2019}
}

@inproceedings{wang2020toward,
title = {Toward few-step adversarial training from a frequency perspective},
author = {Wang, Hans Shih-Han and Cornelius, Cory and Edwards, Brandon and Martin, Jason},
booktitle = {Proceedings of the 1st ACM Workshop on Security and Privacy on Artificial Intelligence},
pages = {11--19},
year = {2020}
}

@inproceedings{madry2017towards,
title = {Towards Deep Learning Models Resistant to Adversarial Attacks},
author = {Aleksander Madry and Aleksandar Makelov and Ludwig Schmidt and Dimitris Tsipras and Adrian Vladu},
booktitle = {ICLR 2018},
year = {2018}
}

@inproceedings{andriushchenko2020understanding,
title = {Understanding and Improving Fast Adversarial Training},
author = {Maksym Andriushchenko and Nicolas Flammarion},
booktitle = {NeurIPS 2020},
year = {2020}
}

@inproceedings{kim2021understanding,
title = {Understanding Catastrophic Overfitting in Single-step Adversarial Training},
author = {Hoki Kim and Woojin Lee and Jaewook Lee},
booktitle = {AAAI 2021},
pages = {8119--8127},
year = {2021}
}

@inproceedings{yu2022understanding,
title = {Understanding Robust Overfitting of Adversarial Training and Beyond},
author = {Chaojian Yu and Bo Han and Li Shen and Jun Yu and Chen Gong and Mingming Gong and Tongliang Liu},
booktitle = {ICML 2022},
volume = {162},
pages = {25595--25610},
year = {2022}
}

@inproceedings{shafahi2020universal,
title = {Universal Adversarial Training},
author = {Ali Shafahi and Mahyar Najibi and Zheng Xu and John P. Dickerson and Larry S. Davis and Tom Goldstein},
booktitle = {AAAI 2020},
pages = {5636--5643},
year = {2020}
}

@inproceedings{benz2021universal,
title = {Universal adversarial training with class-wise perturbations},
author = {Benz, Philipp and Zhang, Chaoning and Karjauv, Adil and Kweon, In So},
booktitle = {ICME 2021},
pages = {1--6},
organization = {IEEE},
year = {2021}
}

@inproceedings{carmon2019unlabeled,
title = {Unlabeled Data Improves Adversarial Robustness},
author = {Yair Carmon and Aditi Raghunathan and Ludwig Schmidt and John C. Duchi and Percy Liang},
booktitle = {NeurIPS 2019},
pages = {11190--11201},
year = {2019}
}

@article{li2023wat,
title = {WAT: Improve the Worst-class Robustness in Adversarial Training},
author = {Li, Boqi and Liu, Weiwei},
journal = {ArXiv preprint},
volume = {abs/2302.04025},
year = {2023}
}

@article{xing2022artificially,
title = {Why Do Artificially Generated Data Help Adversarial Robustness},
author = {Xing, Yue and Song, Qifan and Cheng, Guang},
journal = {Advances in Neural Information Processing Systems},
volume = {35},
pages = {954--966},
year = {2022}
}

@inproceedings{rice2020overfitting,
  title={Overfitting in adversarially robust deep learning},
  author={Rice, Leslie and Wong, Eric and Kolter, Zico},
  booktitle={International Conference on Machine Learning},
  pages={8093--8104},
  year={2020},
  organization={PMLR}
}

@inproceedings{zhang2019you,
title = {You Only Propagate Once: Accelerating Adversarial Training via Maximal Principle},
author = {Dinghuai Zhang and Tianyuan Zhang and Yiping Lu and Zhanxing Zhu and Bin Dong},
booktitle = {NeurIPS 2019},
pages = {227--238},
year = {2019}
}

@inproceedings{dolatabadi2022,
title = {$\ell_{\infty}$-robustness and beyond: Unleashing efficient adversarial training},
author = {Dolatabadi, Hadi M and Erfani, Sarah and Leckie, Christopher},
booktitle = {ECCV 2022},
pages = {467--483},
organization = {Springer},
year = {2022}
}

@article{patil2021robustifying,
title = {Robustifying L∞ Adversarial Training to the Union of Perturbation Models.},
author = {Patil, Ameya D and Tuttle, Michael and Schwing, Alexander G and Shanbhag, Naresh R},
journal = {CoRR},
year = {2021}
}

%=====================================
training-stage defense against backdoor

%=========
%a) Secure centralized training against data-poisoning-based backdoor attack

%=========
%b) Secure decentralized training against partially train-ing controllable backdoor attack

@inproceedings{FedGame_2023,
title = {FedGame: A Game-Theoretic Defense against Backdoor Attacks in Federated Learning},
author = {Jinyuan Jia, Zhuowen Yuan, Dinuka Sahabandu, Luyao Niu, Arezoo Rajabi, Bhaskar Ramasubramanian, Bo Li, Radha Poovendran},
booktitle = {NeurIPS 2023},
year = {2023}
}

@inproceedings{Lockdown_2023,
title = {Lockdown: Backdoor Defense for Federated Learning with Isolated Subspace Training},
author = {Tiansheng Huang, Sihao Hu, Ka-Ho Chow, Fatih Ilhan, Selim Furkan Tekin, Ling Liu},
booktitle = {NeurIPS 2023},
year = {2023}
}

@inproceedings{fedFa_2023,
title = {Fed-FA: Theoretically Modeling Client Data Divergence for Federated Language Backdoor Defense},
author = {Zhiyuan Zhang, Deli Chen, Hao Zhou, Fandong Meng, Jie Zhou, Xu Sun},
booktitle = {NeurIPS 2023},
year = {2023}
}

@InProceedings{Huang_2023_ICCV,
    author    = {Huang, Siquan and Li, Yijiang and Chen, Chong and Shi, Leyu and Gao, Ying},
    title     = {Multi-Metrics Adaptively Identifies Backdoors in Federated Learning},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {4652-4662}
}

@InProceedings{Han_2023_ICCV,
    author    = {Han, Sungwon and Park, Sungwon and Wu, Fangzhao and Kim, Sundong and Zhu, Bin and Xie, Xing and Cha, Meeyoung},
    title     = {Towards Attack-tolerant Federated Learning via Critical Parameter Analysis},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {4999-5008}
}

@article{fung2018mitigating,
title={Mitigating sybils in federated learning poisoning},
author={Fung, Clement and Yoon, Chris JM and Beschastnikh, Ivan},
journal={arXiv preprint arXiv:1808.04866},
year={2018}
}



@inproceedings{xin2023connection,
  title={On the connection between invariant learning and adversarial training for out-of-distribution generalization},
  author={Xin, Shiji and Wang, Yifei and Su, Jingtong and Wang, Yisen},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={37},
  number={9},
  pages={10519--10527},
  year={2023}
}

@inproceedings{yi2021improved,
  title={Improved ood generalization via adversarial training and pretraing},
  author={Yi, Mingyang and Hou, Lu and Sun, Jiacheng and Shang, Lifeng and Jiang, Xin and Liu, Qun and Ma, Zhiming},
  booktitle={International Conference on Machine Learning},
  pages={11987--11997},
  year={2021},
  organization={PMLR}
}

@inproceedings{cao2019understanding,
title={Understanding distributed poisoning attack in federated learning},
author={Cao, Di and Chang, Shan and Lin, Zhijian and Liu, Guohua and Sun, Donghong},
booktitle={2019 IEEE 25th International Conference on Parallel and Distributed Systems (ICPADS)},
pages={233--239},
organization={IEEE},
year={2019}
}

@inproceedings{tolpegin2020data,
title={Data poisoning attacks against federated learning systems},
author={Tolpegin, Vale and Truex, Stacey and Gursoy, Mehmet Emre and Liu, Ling},
booktitle={Computer Security--ESORICS 2020: 25th European Symposium on Research in Computer Security, ESORICS 2020, Guildford, UK, September 14--18, 2020, Proceedings, Part I 25},
pages={480--501},
organization={Springer},
year={2020}
}

@article{li2020learning,
title={Learning to detect malicious clients for robust federated learning},
author={Li, Suyi and Cheng, Yong and Wang, Wei and Liu, Yang and Chen, Tianjian},
journal={arXiv preprint arXiv:2002.00211},
year={2020}
}

@inproceedings{ozdayi2021defending,
title={Defending against backdoors in federated learning with robust learning rate},
author={Ozdayi, Mustafa Safa and Kantarcioglu, Murat and Gel, Yulia R},
booktitle = {AAAI},
volume={35},
pages={9268--9276},
number={10},
year={2021}
}

@inproceedings{xie2021crfl,
title={Crfl: Certifiably robust federated learning against backdoor attacks},
author={Xie, Chulin and Chen, Minghao and Chen, Pin-Yu and Li, Bo},
booktitle = {ICML 2021},
pages={11372--11382},
organization={PMLR},
year={2021}
}

@inproceedings{nguyen2022flame,
title={$\{$FLAME$\}$: Taming backdoors in federated learning},
author={Nguyen, Thien Duc and Rieger, Phillip and De Viti, Roberta and Chen, Huili and Brandenburg, Bj{\o}rn B and Yalame, Hossein and M{\o}llering, Helen and Fereidooni, Hossein and Marchal, Samuel and Miettinen, Markus and others},
booktitle={31st USENIX Security Symposium (USENIX Security 22)},
pages={1415--1432},
year={2022}
}

@inproceedings{hdbscan,
  title={Density-based clustering based on hierarchical density estimates},
  author={Campello, Ricardo JGB and Moulavi, Davoud and Sander, J{\"o}rg},
  booktitle={Pacific-Asia conference on knowledge discovery and data mining},
  pages={160--172},
  year={2013},
  organization={Springer}
}

@article{lu2022defense,
title={Defense against backdoor attack in federated learning},
author={Lu, Shiwei and Li, Ruihu and Liu, Wenbin and Chen, Xuan},
journal={Computers \& Security},
publisher={Elsevier},
volume={121},
pages={102819},
year={2022}
}


@article{gao2022secure,
title={Secure partial aggregation: Making federated learning more robust for industry 4.0 applications},
author={Gao, Jiqiang and Zhang, Baolei and Guo, Xiaojie and Baker, Thar and Li, Min and Liu, Zheli},
journal={IEEE Transactions on Industrial Informatics},
publisher={IEEE},
volume={18},
pages={6340--6348},
number={9},
year={2022}
}

@inproceedings{miao2022against,
title={Against backdoor attacks in federated learning with differential privacy},
author={Miao, Lu and Yang, Wei and Hu, Rong and Li, Lu and Huang, Liusheng},
booktitle = {ICASSP 2022},
pages={2999--3003},
organization={IEEE},
year={2022}
}
@article{cai2022randomized,
  title={Randomized channel shuffling: Minimal-overhead backdoor attack detection without clean datasets},
  author={Cai, Ruisi and Zhang, Zhenyu and Chen, Tianlong and Chen, Xiaohan and Wang, Zhangyang},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={33876--33889},
  year={2022}
}

%-------------------------
% post-training/deployment stage defense 
%-------------------------
% post-training defense zml start 
% defense zml
@inproceedings{liu2018fine,
  title={Fine-pruning: Defending against backdooring attacks on deep neural networks},
  author={Liu, Kang and Dolan-Gavitt, Brendan and Garg, Siddharth},
  booktitle={Research in Attacks, Intrusions, and Defenses: 21st International Symposium, RAID 2018, Heraklion, Crete, Greece, September 10-12, 2018, Proceedings 21},
  pages={273--294},
  year={2018},
  organization={Springer}
}

@inproceedings{wang2019neural,
  title={Neural cleanse: Identifying and mitigating backdoor attacks in neural networks},
  author={Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={707--723},
  year={2019},
  organization={IEEE}
}
@inproceedings{chen2019deepinspect,
  title={Deepinspect: a black-box Trojan detection and mitigation framework for deep neural networks},
  author={Chen, Huili and Fu, Cheng and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={Proceedings of the 28th International Joint Conference on Artificial Intelligence},
  pages={4658--4664},
  year={2019}
}

@article{qiao2019defending,
  title={Defending neural backdoors via generative distribution modeling},
  author={Qiao, Ximing and Yang, Yukun and Li, Hai},
  journal={Advances in neural information processing systems},
  volume={32},
  year={2019}
}

@inproceedings{zhao2020bridging,
  title={BRIDGING MODE CONNECTIVITY IN LOSS LANDSCAPES AND ADVERSARIAL ROBUSTNESS},
  author={Zhao, Pu and Chen, Pin-Yu and Das, Payel and Ramamurthy, Karthikeyan Natesan and Lin, Xue},
  booktitle={International Conference on Learning Representations (ICLR 2020)},
  year={2020}
}

@inproceedings{li2021neural,
title={Neural Attention Distillation: Erasing Backdoor Triggers from Deep Neural Networks},
author={Yige Li and Xixiang Lyu and Nodens Koren and Lingjuan Lyu and Bo Li and Xingjun Ma},
booktitle={International Conference on Learning Representations},
year={2021}
}

@article{wu2021adversarial,
  title={Adversarial neuron pruning purifies backdoored deep models},
  author={Wu, Dongxian and Wang, Yisen},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={16913--16925},
  year={2021}
}

@inproceedings{zheng2022data,
  title={Data-free backdoor removal based on channel lipschitzness},
  author={Zheng, Runkai and Tang, Rongjun and Li, Jianze and Liu, Li},
  booktitle={Computer Vision--ECCV 2022: 17th European Conference, Tel Aviv, Israel, October 23--27, 2022, Proceedings, Part V},
  pages={175--191},
  year={2022},
  organization={Springer}
}
@inproceedings{guan2022few,
  title={Few-shot backdoor defense using shapley estimation},
  author={Guan, Jiyang and Tu, Zhuozhuo and He, Ran and Tao, Dacheng},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13358--13367},
  year={2022}
}
@inproceedings{tao2022better,
  title={Better trigger inversion optimization in backdoor scanning},
  author={Tao, Guanhong and Shen, Guangyu and Liu, Yingqi and An, Shengwei and Xu, Qiuling and Ma, Shiqing and Li, Pan and Zhang, Xiangyu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13368--13378},
  year={2022}
}
@inproceedings{
zeng2022adversarial,
title={Adversarial Unlearning of Backdoors via Implicit Hypergradient},
author={Yi Zeng and Si Chen and Won Park and Zhuoqing Mao and Ming Jin and Ruoxi Jia},
booktitle={International Conference on Learning Representations},
year={2022}
}

@article{zheng2022pre,
  title={Pre-activation Distributions Expose Backdoor Neurons},
  author={Zheng, Runkai and Tang, Rongjun and Li, Jianze and Liu, Li},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={18667--18680},
  year={2022}
}
@article{chai2022one,
  title={One-shot neural backdoor erasing via adversarial weight masking},
  author={Chai, Shuwen and Chen, Jinghui},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  pages={22285--22299},
  year={2022}
}

@inproceedings{zhang2022purifier,
  title={Purifier: Plug-and-play Backdoor Mitigation for Pre-trained Models Via Anomaly Activation Suppression},
  author={Zhang, Xiaoyu and Jin, Yulin and Wang, Tao and Lou, Jian and Chen, Xiaofeng},
  booktitle={Proceedings of the 30th ACM International Conference on Multimedia},
  pages={4291--4299},
  year={2022}
}

@inproceedings{pang2023backdoor,
  title={Backdoor cleansing with unlabeled data},
  author={Pang, Lu and Sun, Tao and Ling, Haibin and Chen, Chao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12218--12227},
  year={2023}
}
@inproceedings{mu2023progressive,
  title={Progressive Backdoor Erasing via connecting Backdoor and Adversarial Attacks},
  author={Mu, Bingxu and Niu, Zhenxing and Wang, Le and Wang, Xue and Miao, Qiguang and Jin, Rong and Hua, Gang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={20495--20503},
  year={2023}
}
@inproceedings{yang2023backdoor,
  title={Backdoor Defense via Suppressing Model Shortcuts},
  author={Yang, Sheng and Li, Yiming and Jiang, Yong and Xia, Shu-Tao},
  booktitle={ICASSP 2023-2023 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={1--5},
  year={2023},
  organization={IEEE}
}

@inproceedings{wang2023unicorn,
  title={UNICORN: A Unified Backdoor Trigger Inversion Framework},
  author={Wang, Zhenting and Mei, Kai and Zhai, Juan and Ma, Shiqing},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2023}
}
@inproceedings{sun2023single,
  title={Single Image Backdoor Inversion via Robust Smoothed Classifiers},
  author={Sun, Mingjie and Kolter, Zico},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8113--8122},
  year={2023}
}

@InProceedings{Zhu_2023_ICCV,
    author    = {Zhu, Mingli and Wei, Shaokui and Shen, Li and Fan, Yanbo and Wu, Baoyuan},
    title     = {Enhancing Fine-Tuning Based Backdoor Defense with Sharpness-Aware Minimization},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {4466-4477}
}



% detection zml
@inproceedings{liu2019abs,
  title={Abs: Scanning neural networks for back-doors by artificial brain stimulation},
  author={Liu, Yingqi and Lee, Wen-Chuan and Tao, Guanhong and Ma, Shiqing and Aafer, Yousra and Zhang, Xiangyu},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={1265--1282},
  year={2019}
}

@inproceedings{shen2021backdoor,
  title={Backdoor scanning for deep neural networks through k-arm optimization},
  author={Shen, Guangyu and Liu, Yingqi and Tao, Guanhong and An, Shengwei and Xu, Qiuling and Cheng, Siyuan and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={International Conference on Machine Learning},
  pages={9525--9536},
  year={2021},
  organization={PMLR}
}
@inproceedings{kolouri2020universal,
  title={Universal litmus patterns: Revealing backdoor attacks in cnns},
  author={Kolouri, Soheil and Saha, Aniruddha and Pirsiavash, Hamed and Hoffmann, Heiko},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={301--310},
  year={2020}
}
@inproceedings{wang2020practical,
  title={Practical Detection of Trojan Neural Networks: Data-Limited and Data-Free Cases},
  author={Wang, Ren and Zhang, Gaoyuan and Liu, Sijia and Chen, Pin-Yu and Xiong, Jinjun and Wang, Meng},
  booktitle={European Conference on Computer Vision},
  pages={222--238},
  year={2020}
}
@inproceedings{huang2020one,
  title={One-Pixel Signature: Characterizing CNN Models for Backdoor Detection},
  author={Huang, Shanjiaoyang and Peng, Weiqi and Jia, Zhiwei and Tu, Zhuowen},
  booktitle={European Conference on Computer Vision},
  pages={326--341},
  year={2020}
}
@inproceedings{fields2021trojan,
  title={Trojan signatures in DNN weights},
  author={Fields, Greg and Samragh, Mohammad and Javaheripi, Mojan and Koushanfar, Farinaz and Javidi, Tara},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={12--20},
  year={2021}
}
@inproceedings{xiang2021red,
  title={L-red: Efficient post-training detection of imperceptible backdoor attacks without access to the training set},
  author={Xiang, Zhen and Miller, David J and Kesidis, George},
  booktitle={ICASSP 2021-2021 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)},
  pages={3745--3749},
  year={2021},
  organization={IEEE}
}

@inproceedings{xu2021detecting,
  title={Detecting ai trojans using meta neural analysis},
  author={Xu, Xiaojun and Wang, Qi and Li, Huichen and Borisov, Nikita and Gunter, Carl A and Li, Bo},
  booktitle={2021 IEEE Symposium on Security and Privacy (SP)},
  pages={103--120},
  year={2021},
  organization={IEEE}
}

@inproceedings{hu2022trigger,
  title={Trigger Hunting with a Topological Prior for Trojan Detection},
  author={Hu, Xiaoling and Lin, Xiao and Cogswell, Michael and Yao, Yi and Jha, Susmit and Chen, Chao},
  booktitle={International Conference on Learning Representations},
  year={2022}
}
@inproceedings{guo2022aeva,
  title={AEVA: Black-box Backdoor Detection Using Adversarial Extreme Value Analysis},
  author={Guo, Junfeng and Li, Ang and Liu, Cong},
  booktitle={International Conference on Learning Representations},
  year={2022}
}
@inproceedings{xiang2022post,
  title={Post-Training Detection of Backdoor Attacks for Two-Class and Multi-Attack Scenarios},
  author={Xiang, Zhen and Miller, David and Kesidis, George},
  booktitle={International Conference on Learning Representations},
  year={2022}
}
@inproceedings{feng2023detecting,
  title={Detecting Backdoors in Pre-trained Encoders},
  author={Feng, Shiwei and Tao, Guanhong and Cheng, Siyuan and Shen, Guangyu and Xu, Xiangzhe and Liu, Yingqi and Zhang, Kaiyuan and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16352--16362},
  year={2023}
}

@inproceedings{liu2022complex,
  title={Complex backdoor detection by symmetric feature differencing},
  author={Liu, Yingqi and Shen, Guangyu and Tao, Guanhong and Wang, Zhenting and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15003--15013},
  year={2022}
}

@inproceedings{
zhu2023neural,
title={Neural Polarizer: A Lightweight and Effective Backdoor Defense via Purifying Poisoned Features},
author={Mingli Zhu and Shaokui Wei and Hongyuan Zha and Baoyuan Wu},
booktitle={Thirty-seventh Conference on Neural Information Processing Systems},
year={2023}
}



% post-training defense zml end

%---------- deployment stage defense for (targeted) weight attack
@inproceedings{ozdenizci2022improving,
  title={Improving robustness against stealthy weight bit-flip attacks by output code matching},
  author={{\"O}zdenizci, Ozan and Legenstein, Robert},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13388--13397},
  year={2022}
}

@inproceedings{wang2023aegis,
  title={Aegis: Mitigating Targeted Bit-flip Attacks against Deep Neural Networks},
  author={Wang, Jialai and Zhang, Ziyuan and Wang, Meiqi and Qiu, Han and Zhang, Tianwei and Li, Qi and Li, Zongpeng and Wei, Tao and Zhang, Chao},
  booktitle={USENIX Security Symposium},
  year={2023}
}

@article{liu2023generating,
  title={Generating Robust DNN with Resistance to Bit-Flip based Adversarial Weight Attack},
  author={Liu, Liang and Guo, Yanan and Cheng, Yueqiang and Zhang, Youtao and Yang, Jun},
  journal={IEEE Transactions on Computers},
  year={2023},
  publisher={IEEE}
}

@inproceedings{chen2019deepattest,
  title={DeepAttest: An end-to-end attestation framework for deep neural networks},
  author={Chen, Huili and Fu, Cheng and Rouhani, Bita Darvish and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={Proceedings of the 46th International Symposium on Computer Architecture},
  pages={487--498},
  year={2019}
}


% ================================ post-training backdoor defense================================================
%1-20
@article{ac,
  title={Detecting backdoor attacks on deep neural networks by activation clustering},
  author={Chen, Bryant and Carvalho, Wilka and Baracaldo, Nathalie and Ludwig, Heiko and Edwards, Benjamin and Lee, Taesung and Molloy, Ian and Srivastava, Biplav},
  journal={arXiv preprint arXiv:1811.03728},
  year={2018}
}

@article{spectral,
  title={Spectral signatures in backdoor attacks},
  author={Tran, Brandon and Li, Jerry and Madry, Aleksander},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{Fine-pruning,
  title={Fine-pruning: Defending against backdooring attacks on deep neural networks},
  author={Liu, Kang and Dolan-Gavitt, Brendan and Garg, Siddharth},
  booktitle={Research in Attacks, Intrusions, and Defenses: 21st International Symposium, RAID 2018, Heraklion, Crete, Greece, September 10-12, 2018, Proceedings 21},
  pages={273--294},
  year={2018},
  organization={Springer}
}

@article{neuroninspect,
  title={Neuroninspect: Detecting backdoors in neural networks via output explanations},
  author={Huang, Xijie and Alzantot, Moustafa and Srivastava, Mani},
  journal={arXiv preprint arXiv:1911.07399},
  year={2019}
}

@article{neo,
  title={Model agnostic defence against backdoor attacks in machine learning},
  author={Udeshi, Sakshi and Peng, Shanshan and Woo, Gerald and Loh, Lionell and Rawshan, Louth and Chattopadhyay, Sudipta},
  journal={IEEE Transactions on Reliability},
  volume={71},
  number={2},
  pages={880--895},
  year={2022},
  publisher={IEEE}
}

@inproceedings{abs,
  title={Abs: Scanning neural networks for back-doors by artificial brain stimulation},
  author={Liu, Yingqi and Lee, Wen-Chuan and Tao, Guanhong and Ma, Shiqing and Aafer, Yousra and Zhang, Xiangyu},
  booktitle={Proceedings of the 2019 ACM SIGSAC Conference on Computer and Communications Security},
  pages={1265--1282},
  year={2019}
}

@inproceedings{k-arm,
  title={Backdoor scanning for deep neural networks through k-arm optimization},
  author={Shen, Guangyu and Liu, Yingqi and Tao, Guanhong and An, Shengwei and Xu, Qiuling and Cheng, Siyuan and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={International Conference on Machine Learning},
  pages={9525--9536},
  year={2021},
  organization={PMLR}
}

@inproceedings{nc,
  title={Neural cleanse: Identifying and mitigating backdoor attacks in neural networks},
  author={Wang, Bolun and Yao, Yuanshun and Shan, Shawn and Li, Huiying and Viswanath, Bimal and Zheng, Haitao and Zhao, Ben Y},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={707--723},
  year={2019},
  organization={IEEE}
}

@inproceedings{deepinspect,
  title={DeepInspect: A Black-box Trojan Detection and Mitigation Framework for Deep Neural Networks.},
  author={Chen, Huili and Fu, Cheng and Zhao, Jishen and Koushanfar, Farinaz},
  booktitle={IJCAI},
  volume={2},
  number={5},
  pages={8},
  year={2019}
}

@article{xu2020defending,
  title={Defending against backdoor attack on deep neural networks},
  author={Xu, Kaidi and Liu, Sijia and Chen, Pin-Yu and Zhao, Pu and Lin, Xue},
  journal={arXiv preprint arXiv:2002.12162},
  year={2020}
}



@inproceedings{gangsweep,
  title={Gangsweep: Sweep out neural backdoors by gan},
  author={Zhu, Liuwan and Ning, Rui and Wang, Cong and Xin, Chunsheng and Wu, Hongyi},
  booktitle={Proceedings of the 28th ACM International Conference on Multimedia},
  pages={3173--3181},
  year={2020}
}

@inproceedings{nnoculation,
  title={NNoculation: Catching BadNets in the wild},
  author={Veldanda, Akshaj Kumar and Liu, Kang and Tan, Benjamin and Krishnamurthy, Prashanth and Khorrami, Farshad and Karri, Ramesh and Dolan-Gavitt, Brendan and Garg, Siddharth},
  booktitle={Proceedings of the 14th ACM Workshop on Artificial Intelligence and Security},
  pages={49--60},
  year={2021}
}

@inproceedings{harikumar2021scalable,
  title={Scalable backdoor detection in neural networks},
  author={Harikumar, Haripriya and Le, Vuong and Rana, Santu and Bhattacharya, Sourangshu and Gupta, Sunil and Venkatesh, Svetha},
  booktitle={Machine Learning and Knowledge Discovery in Databases: European Conference, ECML PKDD 2020, Ghent, Belgium, September 14--18, 2020, Proceedings, Part II},
  pages={289--304},
  year={2021},
  organization={Springer}
}

@article{Neural_Network_Laundering,
  title={Neural network laundering: Removing black-box backdoor watermarks from deep neural networks},
  author={Aiken, William and Kim, Hyoungshick and Woo, Simon and Ryoo, Jungwoo},
  journal={Computers \& Security},
  volume={106},
  pages={102277},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{ulp,
  title={Universal litmus patterns: Revealing backdoor attacks in cnns},
  author={Kolouri, Soheil and Saha, Aniruddha and Pirsiavash, Hamed and Hoffmann, Heiko},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={301--310},
  year={2020}
}

@inproceedings{one-pixel,
  title={One-pixel signature: Characterizing cnn models for backdoor detection},
  author={Huang, Shanjiaoyang and Peng, Weiqi and Jia, Zhiwei and Tu, Zhuowen},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XXVII 16},
  pages={326--341},
  year={2020},
  organization={Springer}
}



@inproceedings{tabor,
  title={Towards inspecting and eliminating trojan backdoors in deep neural networks},
  author={Guo, Wenbo and Wang, Lun and Xu, Yan and Xing, Xinyu and Du, Min and Song, Dawn},
  booktitle={2020 IEEE International Conference on Data Mining (ICDM)},
  pages={162--171},
  year={2020},
  organization={IEEE}
}

@article{mcr,
  title={Bridging mode connectivity in loss landscapes and adversarial robustness},
  author={Zhao, Pu and Chen, Pin-Yu and Das, Payel and Ramamurthy, Karthikeyan Natesan and Lin, Xue},
  journal={arXiv preprint arXiv:2005.00060},
  year={2020}
}

% 21-40


@inproceedings{sentinet,
  title={Sentinet: Detecting localized universal attacks against deep learning systems},
  author={Chou, Edward and Tramer, Florian and Pellegrino, Giancarlo},
  booktitle={2020 IEEE Security and Privacy Workshops (SPW)},
  pages={48--54},
  year={2020},
  organization={IEEE}
}

@article{xiang2020detection,
  title={Detection of backdoors in trained classifiers without access to the training set},
  author={Xiang, Zhen and Miller, David J and Kesidis, George},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  volume={33},
  number={3},
  pages={1177--1191},
  year={2020},
  publisher={IEEE}
}

@article{sikka2020detecting,
  title={Detecting trojaned dnns using counterfactual attributions},
  author={Sikka, Karan and Sur, Indranil and Jha, Susmit and Roy, Anirban and Divakaran, Ajay},
  journal={arXiv preprint arXiv:2012.02275},
  year={2020}
}

@article{ex-ray,
  title={Ex-ray: Distinguishing injected backdoor from natural features in neural networks by examining differential feature symmetry},
  author={Liu, Yingqi and Shen, Guangyu and Tao, Guanhong and Wang, Zhenting and Ma, Shiqing and Zhang, Xiangyu},
  journal={arXiv preprint arXiv:2103.08820},
  year={2021}
}

@article{ntd,
  title={NTD: Non-Transferability Enabled Backdoor Detection},
  author={Li, Yinshan and Ma, Hua and Zhang, Zhi and Gao, Yansong and Abuadbba, Alsharif and Fu, Anmin and Zheng, Yifeng and Al-Sarawi, Said F and Abbott, Derek},
  journal={arXiv preprint arXiv:2111.11157},
  year={2021}
}

@article{sun2021general,
  title={A general framework for defending against backdoor attacks via influence graph},
  author={Sun, Xiaofei and Li, Jiwei and Li, Xiaoya and Wang, Ziyao and Zhang, Tianwei and Qiu, Han and Wu, Fei and Fan, Chun},
  journal={arXiv preprint arXiv:2111.14309},
  year={2021}
}

@article{tad,
  title={Tad: Trigger approximation based black-box trojan detection for ai},
  author={Zhang, Xinqiao and Chen, Huili and Koushanfar, Farinaz},
  journal={arXiv preprint arXiv:2102.01815},
  year={2021}
}

@article{top,
  title={Top: Backdoor detection in neural networks via transferability of perturbation},
  author={Huster, Todd and Ekwedike, Emmanuel},
  journal={arXiv preprint arXiv:2103.10274},
  year={2021}
}


@inproceedings{zeng2021rethinking,
  title={Rethinking the backdoor attacks' triggers: A frequency perspective},
  author={Zeng, Yi and Park, Won and Mao, Z Morley and Jia, Ruoxi},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={16473--16481},
  year={2021}
}


@inproceedings{
nad,
title={Neural Attention Distillation: Erasing Backdoor Triggers from Deep Neural Networks},
author={Yige Li and Xixiang Lyu and Nodens Koren and Lingjuan Lyu and Bo Li and Xingjun Ma},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=9l0K4OM-oXE}
}

@article{fan2022defense,
  title={Defense against Backdoor Attacks via Identifying and Purifying Bad Neurons},
  author={Fan, Mingyuan and Liu, Yang and Chen, Cen and Liu, Ximeng and Guo, Wenzhong},
  journal={arXiv preprint arXiv:2208.06537},
  year={2022}
}

@misc{bajcsy2021baseline,
      title={Baseline Pruning-Based Approach to Trojan Detection in Neural Networks}, 
      author={Peter Bajcsy and Michael Majurski},
      year={2021},
      eprint={2101.12016},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@inproceedings{spectre,
  title={Spectre: Defending against backdoor attacks using robust covariance estimation},
  author={Hayase, Jonathan and Kong, Weihao},
  booktitle={International Conference on Machine Learning},
  year={2021}
}

@inproceedings{liu2021removing,
  title={Removing Backdoor-Based Watermarks in Neural Networks with Limited Data},
  author={Liu, Xuankai and Li, Fengting and Wen, Bihan and Li, Qi},
  booktitle={2020 25th International Conference on Pattern Recognition (ICPR)},
  pages={10149--10156},
  year={2021},
  organization={IEEE Computer Society}
}



@article{odyssey,
  title={Odyssey: Creation, analysis and detection of trojan models},
  author={Edraki, Marzieh and Karim, Nazmul and Rahnavard, Nazanin and Mian, Ajmal and Shah, Mubarak},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={16},
  pages={4521--4533},
  year={2021},
  publisher={IEEE}
}

@inproceedings{sun2021detect,
  title={Detect and Remove Watermark in Deep Neural Networks via Generative Adversarial Networks},
  author={Sun, Shichang and Wang, Haoqi and Xue, Mingfu and Zhang, Yushu and Wang, Jian and Liu, Weiqiang},
  booktitle={Information Security: 24th International Conference, ISC 2021, Virtual Event, November 10--12, 2021, Proceedings},
  pages={341--357},
  year={2021}
}

@article{anp,
  title={Adversarial neuron pruning purifies backdoored deep models},
  author={Wu, Dongxian and Wang, Yisen},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={16913--16925},
  year={2021}
}

% 41-60
@article{zheng2021topological,
  title={Topological detection of trojaned neural networks},
  author={Zheng, Songzhu and Zhang, Yikai and Wagner, Hubert and Goswami, Mayank and Chen, Chao},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={17258--17272},
  year={2021}
}

@inproceedings{tang2021demon,
  title={Demon in the Variant: Statistical Analysis of DNNs for Robust Backdoor Contamination Detection.},
  author={Tang, Di and Wang, XiaoFeng and Tang, Haixu and Zhang, Kehuan},
  booktitle={USENIX Security Symposium},
  pages={1541--1558},
  year={2021}
}

@article{UnivBM,
  title={Universal Post-Training Backdoor Detection},
  author={Wang, Hang and Xiang, Zhen and Miller, David J and Kesidis, George},
  journal={arXiv e-prints},
  pages={arXiv--2205},
  year={2022}
}

@article{TrojDef,
  title={An Adaptive Black-Box Defense Against Trojan Attacks (TrojDef)},
  author={Liu, Guanxiong and Khreishah, Abdallah and Sharadgah, Fatima and Khalil, Issa},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}


@misc{A2P,
      title={Universal Backdoor Attacks Detection via Adaptive Adversarial Probe}, 
      author={Yuhang Wang and Huafeng Shi and Rui Min and Ruijia Wu and Siyuan Liang and Yichao Wu and Ding Liang and Aishan Liu},
      year={2022},
      eprint={2209.05244},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@article{MTD,
  title={Defense Against Multi-target Trojan Attacks},
  author={Harikumar, Haripriya and Rana, Santu and Do, Kien and Gupta, Sunil and Zong, Wei and Susilo, Willy and Venkastesh, Svetha},
  journal={arXiv preprint arXiv:2207.03895},
  year={2022}
}

@article{MCLDef,
  title={Model-Contrastive Learning for Backdoor Defense},
  author={Yue, Zhihao and Xia, Jun and Ling, Zhiwei and Wang, Ting and Wei, Xian and Chen, Mingsong},
  journal={arXiv preprint arXiv:2205.04411},
  year={2022}
}

@article{Pidan,
  title={Pidan: a coherence optimization approach for backdoor attack detection and mitigation in deep neural networks},
  author={Wang, Yue and Li, Wenqing and Sarkar, Esha and Shafique, Muhammad and Maniatakos, Michail and Jabari, Saif Eddin},
  journal={arXiv preprint arXiv:2203.09289},
  year={2022}
}



@inproceedings{EX-RAY,
  title={Complex backdoor detection by symmetric feature differencing},
  author={Liu, Yingqi and Shen, Guangyu and Tao, Guanhong and Wang, Zhenting and Ma, Shiqing and Zhang, Xiangyu},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={15003--15013},
  year={2022}
}

@inproceedings{AEVA,
  title={AEVA: Black-box Backdoor Detection Using Adversarial Extreme Value Analysis},
  author={Guo, Junfeng and Li, Ang and Liu, Cong},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@inproceedings{hutrigger,
  title={Trigger Hunting with a Topological Prior for Trojan Detection},
  author={Hu, Xiaoling and Lin, Xiao and Cogswell, Michael and Yao, Yi and Jha, Susmit and Chen, Chao},
  booktitle={International Conference on Learning Representations},
  year={2022}
}

@inproceedings{BAERASER,
  title={Backdoor defense with machine unlearning},
  author={Liu, Yang and Fan, Mingyuan and Chen, Cen and Liu, Ximeng and Ma, Zhuo and Wang, Li and Ma, Jianfeng},
  booktitle={IEEE INFOCOM 2022-IEEE Conference on Computer Communications},
  pages={280--289},
  year={2022},
  organization={IEEE}
}

@article{LinkBreaker,
  title={LinkBreaker: Breaking the Backdoor-Trigger Link in DNNs via Neurons Consistency Check},
  author={Chen, Zhenzhu and Wang, Shang and Fu, Anmin and Gao, Yansong and Yu, Shui and Deng, Robert H},
  journal={IEEE Transactions on Information Forensics and Security},
  volume={17},
  pages={2000--2014},
  year={2022},
  publisher={IEEE}
}

@inproceedings{wang2022trap,
  title={Trap and Replace: Defending Backdoor Attacks by Trapping Them into an Easy-to-Replace Subnetwork},
  author={Wang, Haotao and Hong, Junyuan and Zhang, Aston and Zhou, Jiayu and Wang, Zhangyang},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022},
}

@inproceedings{AWM,
  title={One-shot Neural Backdoor Erasing via Adversarial Weight Masking},
  author={Chai, Shuwen and Chen, Jinghui},
  booktitle={Advances in Neural Information Processing Systems},
  year={2022},
}

@inproceedings{unnervik2022anomaly,
  title={An anomaly detection approach for backdoored neural networks: face recognition as a case study},
  author={Unnervik, Alexander and Marcel, S{\'e}bastien},
  booktitle={2022 International Conference of the Biometrics Special Interest Group (BIOSIG)},
  pages={1--5},
  year={2022},
  organization={IEEE}
}

@article{jiang2022critical,
  title={Critical Path-Based Backdoor Detection for Deep Neural Networks},
  author={Jiang, Wei and Wen, Xiangyu and Zhan, Jinyu and Wang, Xupeng and Song, Ziwei and Bian, Chen},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2022},
  publisher={IEEE}
}

@inproceedings{SCALE-UP,
  title={SCALE-UP: An Efficient Black-box Input-level Backdoor Detection via Analyzing Scaled Prediction Consistency},
  author={Guo, Junfeng and Li, Yiming and Chen, Xun and Guo, Hanqing and Sun, Lichao and Liu, Cong},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2023}
}

@inproceedings{UNICORN,
  title={UNICORN: A Unified Backdoor Trigger Inversion Framework},
  author={Wang, Zhenting and Mei, Kai and Zhai, Juan and Ma, Shiqing},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2023}
}
% ==================================================================================================================
% ================================ secure-training backdoor defense================================================
% secure training defense
% centralized control
@inproceedings{cbd,
  title={Backdoor Defense via Deconfounded Representation Learning},
  author={Zhang, Zaixi and Liu, Qi and Wang, Zhicai and Lu, Zepu and Hu, Qingyong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12228--12238},
  year={2023}
}

@inproceedings{asd,
  title={Backdoor Defense via Adaptively Splitting Poisoned Dataset},
  author={Gao, Kuofeng and Bai, Yang and Gu, Jindong and Yang, Yong and Xia, Shu-Tao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4005--4014},
  year={2023}
}

@article{li2021anti,
  title={Anti-backdoor learning: Training clean models on poisoned data},
  author={Li, Yige and Lyu, Xixiang and Koren, Nodens and Lyu, Lingjuan and Li, Bo and Ma, Xingjun},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  year={2021}
}
@inproceedings{dbd,
  title     = {Backdoor Defense via Decoupling the Training Process},
  author    = {Kunzhe, Huang and Yiming, Li and Baoyuan, Wu and Zhan, Qin and Kui, Ren},
  booktitle = {The Tenth International Conference on Learning Representations},
  year      = {2022}
}

@article{chen2022effective,
  title={Effective backdoor defense by exploiting sensitivity of poisoned samples},
  author={Chen, Weixin and Wu, Baoyuan and Wang, Haoqian},
  journal={Advances in Neural Information Processing Systems},
  volume={35},
  year={2022}
}

@inproceedings{gao2023backdoor,
  title={Backdoor Defense via Adaptively Splitting Poisoned Dataset},
  author={Gao, Kuofeng and Bai, Yang and Gu, Jindong and Yang, Yong and Xia, Shu-Tao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={4005--4014},
  year={2023}
}

@inproceedings{zhang2023backdoor,
  title={Backdoor Defense via Deconfounded Representation Learning},
  author={Zhang, Zaixi and Liu, Qi and Wang, Zhicai and Lu, Zepu and Hu, Qingyong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12228--12238},
  year={2023}
}



@inproceedings{weber2022rab,
  title={RAB: Provable Robustness Against Backdoor Attacks},
  author={Weber, Maurice and Xu, Xiaojun and Karlas, Bojan and Zhang, Ce and Li, Bo},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={640--657},
  year={2022},
  organization={IEEE Computer Society}
}

@article{ali2020has,
  title={Has-nets: A heal and select mechanism to defend dnns against backdoor attacks for data collection scenarios},
  author={Ali, Hassan and Nepal, Surya and Kanhere, Salil S and Jha, Sanjay},
  journal={arXiv preprint arXiv:2012.07474},
  year={2020}
}

@article{hong2020effectiveness,
  title={On the effectiveness of mitigating data poisoning attacks with gradient shaping},
  author={Hong, Sanghyun and Chandrasekaran, Varun and Kaya, Yi{\u{g}}itcan and Dumitra{\c{s}}, Tudor and Papernot, Nicolas},
  journal={arXiv preprint arXiv:2002.11497},
  year={2020}
}
@article{soremekun2020exposing,
  title={Exposing backdoors in robust machine learning models},
  author={Soremekun, Ezekiel and Udeshi, Sakshi and Chattopadhyay, Sudipta},
  journal={arXiv preprint arXiv:2003.00865},
  year={2020}
}

@article{gao2023effectiveness,
  title={On the effectiveness of adversarial training against backdoor attacks},
  author={Gao, Yinghua and Wu, Dongxian and Zhang, Jingfeng and Gan, Guanhao and Xia, Shu-Tao and Niu, Gang and Sugiyama, Masashi},
  journal={IEEE Transactions on Neural Networks and Learning Systems},
  year={2023},
  publisher={IEEE}
}

@article{weng2020trade,
  title={On the trade-off between adversarial and backdoor robustness},
  author={Weng, Cheng-Hsin and Lee, Yan-Ting and Wu, Shan-Hung Brandon},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={11973--11983},
  year={2020}
}
@inproceedings{jia2021intrinsic,
  title={Intrinsic certified robustness of bagging against data poisoning attacks},
  author={Jia, Jinyuan and Cao, Xiaoyu and Gong, Neil Zhenqiang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={35},
  number={9},
  pages={7961--7969},
  year={2021}
}
@article{wang2022pidan,
  title={Pidan: a coherence optimization approach for backdoor attack detection and mitigation in deep neural networks},
  author={Wang, Yue and Li, Wenqing and Sarkar, Esha and Shafique, Muhammad and Maniatakos, Michail and Jabari, Saif Eddin},
  journal={arXiv preprint arXiv:2203.09289},
  year={2022}
}

@inproceedings{dong2021black,
  title={Black-box detection of backdoor attacks with limited information and data},
  author={Dong, Yinpeng and Yang, Xiao and Deng, Zhijie and Pang, Tianyu and Xiao, Zihao and Su, Hang and Zhu, Jun},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={16482--16491},
  year={2021}
}
@inproceedings{DPA,
  author={Alexander Levine and Soheil Feizi},
  title     = {Deep Partition Aggregation: Provable Defenses against General Poisoning Attacks},
  booktitle = {9th International Conference on Learning Representations, {ICLR} 2021, Virtual Event, Austria, May 3-7, 2021},
  year      = {2021}
}
@inproceedings{jia2022certified,
  title={Certified robustness of nearest neighbors against data poisoning and backdoor attacks},
  author={Jia, Jinyuan and Liu, Yupei and Cao, Xiaoyu and Gong, Neil Zhenqiang},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  pages={9575--9583},
  year={2022}
}

@article{zhang2022bagflip,
  title={BagFlip: A Certified Defense against Data Poisoning},
  author={Yuhao Zhang, Aws Albarghouthi, Loris D'Antoni},
  journal={Advances in Neural Information Processing Systems},
  year={2022}
}

@article{hou2022similarity,
  title={Similarity-based integrity protection for deep learning systems},
  author={Hou, Ruitao and Ai, Shan and Chen, Qi and Yan, Hongyang and Huang, Teng and Chen, Kongyang},
  journal={Information Sciences},
  pages={255--267},
  year={2022},
}

@inproceedings{qi2022fight,
  title={Fight poison with poison: Detecting backdoor poison samples via decoupling benign correlations},
  author={Qi, Xiangyu and Xie, Tinghao and Mahloujifar, Saeed and Mittal, Prateek},
  booktitle={USENIX Security Symposium},
  year={2023}
}

% partial control


@inproceedings{cheng2023beagle,
  title={{BEAGLE:} Forensics of Deep Learning Backdoor Attack for Better Defense},
  author = {Cheng, Siyuan and Tao, Guanhong and Liu, Yingqi and An, Shengwei and Xu, Xiangzhe and Feng, Shiwei and Shen, Guangyu and Zhang, Kaiyuan and Xu, Qiuling and Ma, Shiqing and others},
  booktitle = {30th Annual Network and Distributed System Security Symposium},
  year = {2023}
}

@inproceedings{zhang2022flip,
  title={FLIP: A Provable Defense Framework for Backdoor Mitigation in Federated Learning},
  author={Zhang, Kaiyuan and Tao, Guanhong and Xu, Qiuling and Cheng, Siyuan and An, Shengwei and Liu, Yingqi and Feng, Shiwei and Shen, Guangyu and Chen, Pin-Yu and Ma, Shiqing and others},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2023}
}

@article{sun2019can,
 author = {Sun, Ziteng and Kairouz, Peter and Suresh, Ananda Theertha and McMahan, H Brendan},
 journal = {ArXiv preprint},
 title = {Can you really backdoor federated learning?},
 year = {2019}
}

@article{lin2023mitigating,
 author = {Lin, Yihang and Zhou, Pengyuan and Wu, Zhiqian and Liao, Yong},
 journal = {ArXiv preprint},
 title = {Mitigating Backdoors in Federated Learning with FLD},
 year = {2023}
}

@article{rodriguez2022backdoor,
  title={Backdoor attacks-resilient aggregation based on Robust Filtering of Outliers in federated learning for image classification},
  author={Rodr{\'\i}guez-Barroso, Nuria and Mart{\'\i}nez-C{\'a}mara, Eugenio and Luz{\'o}n, M Victoria and Herrera, Francisco},
  journal={Knowledge-Based Systems},
  volume={245},
  pages={108588},
  year={2022},
  publisher={Elsevier}
}

@article{liu2023evil,
  title = {Evil vs evil: using adversarial examples to against backdoor attack in federated learning},
 author = {Liu, Tao and Li, Mingjun and Zheng, Haibin and Ming, Zhaoyan and Chen, Jinyin},
 journal = {Multimedia Systems},
 pages = {553--568},
 year = {2023}
}

@article{jebreel2023fl,
 title = {FL-Defender: Combating targeted attacks in federated learning},
 author = {Jebreel, Najeeb Moharram and Domingo-Ferrer, Josep},
 journal = {Knowledge-Based Systems},
 pages = {110178},
 year = {2023}
}

@article{hallaji2023label,
 title = {Label noise analysis meets adversarial training: A defense against label poisoning in federated learning},
 author = {Hallaji, Ehsan and Razavi-Far, Roozbeh and Saif, Mehrdad and Herrera-Viedma, Enrique},
 journal = {Knowledge-Based Systems},
 pages = {110384},
 publisher = {Elsevier},
 year = {2023}
}

@article{blanchard2017machine,
  title={Machine learning with adversaries: Byzantine tolerant gradient descent},
  author={Blanchard, Peva and El Mhamdi, El Mahdi and Guerraoui, Rachid and Stainer, Julien},
  journal={Advances in neural information processing systems},
  volume={30},
  year={2017}
}

@article{pillutla2022robust,
 title = {Robust aggregation for federated learning},
 author = {Pillutla, Krishna and Kakade, Sham M and Harchaoui, Zaid},
 journal = {IEEE Transactions on Signal Processing},
 pages = {1142--1154},
 year = {2022}
}

@inproceedings{rieger2022deepsight,
 author = {Rieger, Phillip and Nguyen, Thien Duc and Miettinen, Markus and Sadeghi, Ahmad-Reza},
 title = {Deepsight: Mitigating backdoor attacks in federated learning through deep model inspection},
 booktitle  = {29th Annual Network and Distributed System Security Symposium},
 year = {2022}
}

@inproceedings{xie2021crfl,
  title={Crfl: Certifiably robust federated learning against backdoor attacks},
  author={Xie, Chulin and Chen, Minghao and Chen, Pin-Yu and Li, Bo},
  booktitle={International Conference on Machine Learning},
  pages={11372--11382},
  year={2021},
  organization={PMLR}
}

@inproceedings{bagdasaryan2020backdoor,
  title={How to backdoor federated learning},
  author={Bagdasaryan, Eugene and Veit, Andreas and Hua, Yiqing and Estrin, Deborah and Shmatikov, Vitaly},
  booktitle={International conference on artificial intelligence and statistics},
  pages={2938--2948},
  year={2020},
  organization={PMLR}
}


@inproceedings{xie2019dba,
  title={Dba: Distributed backdoor attacks against federated learning},
  author={Xie, Chulin and Huang, Keli and Chen, Pin-Yu and Li, Bo},
  booktitle={International conference on learning representations},
  year={2019}
}

@article{wang2020attack,
  title={Attack of the tails: Yes, you really can backdoor federated learning},
  author={Wang, Hongyi and Sreenivasan, Kartik and Rajput, Shashank and Vishwakarma, Harit and Agarwal, Saurabh and Sohn, Jy-yong and Lee, Kangwook and Papailiopoulos, Dimitris},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={16070--16084},
  year={2020}
}

%==========================================================================================================
%  Defense against inference-time adversarial defense
% denoising/purification
@inproceedings{liu2019feature,
  title={Feature distillation: Dnn-oriented jpeg compression against adversarial examples},
  author={Liu, Zihao and Liu, Qi and Liu, Tao and Xu, Nuo and Lin, Xue and Wang, Yanzhi and Wen, Wujie},
  booktitle={CVPR},
  pages={860--868},
  year={2019},
  organization={IEEE}
}

@inproceedings{naseer2020self,
  title={A self-supervised approach for adversarial robustness},
  author={Naseer, Muzammal and Khan, Salman and Hayat, Munawar and Khan, Fahad Shahbaz and Porikli, Fatih},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={262--271},
  year={2020}
}

@article{das2017keeping,
  title={Keeping the bad guys out: Protecting and vaccinating deep learning with jpeg compression},
  author={Das, Nilaksh and Shanbhogue, Madhuri and Chen, Shang-Tse and Hohman, Fred and Chen, Li and Kounavis, Michael E and Chau, Duen Horng},
  journal={arXiv preprint arXiv:1705.02900},
  year={2017}
}

@inproceedings{das2018shield,
  title={SHIELD: Fast, Practical Defense and Vaccination for Deep Learning using JPEG Compression},
  author={Das, Nilaksh and Shanbhogue, Madhuri and Chen, Shang-Tse and Hohman, Fred and Li, Siwei and Chen, Li and Kounavis, Michael E and Chau, Duen Horng},
  booktitle={ACM SIGKDD Conference on Knowledge Discovery and Data Mining},
  year={2018}
}

@article{song2018defense,
  title={Defense against adversarial attacks with saak transform},
  author={Song, Sibo and Chen, Yueru and Cheung, Ngai-Man and Kuo, C-C Jay},
  journal={arXiv preprint arXiv:1808.01785},
  year={2018}
}

@article{mustafa2019image,
  title={Image super-resolution as a defense against adversarial attacks},
  author={Mustafa, Aamir and Khan, Salman H and Hayat, Munawar and Shen, Jianbing and Shao, Ling},
  journal={IEEE Transactions on Image Processing},
  volume={29},
  pages={1711--1724},
  year={2019},
  publisher={IEEE}
}

@article{salman2020denoised,
  title={Denoised smoothing: A provable defense for pretrained classifiers},
  author={Salman, Hadi and Sun, Mingjie and Yang, Greg and Kapoor, Ashish and Kolter, J Zico},
  journal={NeurIPS},
  volume={33},
  pages={21945--21957},
  year={2020}
}

@inproceedings{chen2022adversarial,
  title={Adversarial Attack on Attackers: Post-Process to Mitigate Black-Box Score-Based Query Attacks},
  author={Chen, Sizhe and Huang, Zhehao and Tao, Qinghua and Wu, Yingwen and Xie, Cihang and Huang, Xiaolin},
  booktitle={NeurIPS},
  year={2022}
}

@inproceedings{guocountering,
  title={Countering Adversarial Images using Input Transformations},
  author={Guo, Chuan and Rana, Mayank and Cisse, Moustapha and van der Maaten, Laurens},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{meng2017magnet,
  title={Magnet: a two-pronged defense against adversarial examples},
  author={Meng, Dongyu and Chen, Hao},
  booktitle={Proceedings of the 2017 ACM SIGSAC conference on computer and communications security},
  pages={135--147},
  year={2017}
}

@inproceedings{liao2018defense,
  title={Defense against adversarial attacks using high-level representation guided denoiser},
  author={Liao, Fangzhou and Liang, Ming and Dong, Yinpeng and Pang, Tianyu and Hu, Xiaolin and Zhu, Jun},
  booktitle={CVPR},
  pages={1778--1787},
  year={2018}
}

@article{moosavi2018divide,
  title={Divide, denoise, and defend against adversarial attacks},
  author={Moosavi-Dezfooli, Seyed-Mohsen and Shrivastava, Ashish and Tuzel, Oncel},
  booktitle={CVPR},
  year={2018}
}

@inproceedings{alfarra2022combating,
  title={Combating adversaries with anti-adversaries},
  author={Alfarra, Motasem and P{\'e}rez, Juan C and Thabet, Ali and Bibi, Adel and Torr, Philip HS and Ghanem, Bernard},
  booktitle={AAAI},
  volume={36},
  pages={5992--6000},
  year={2022}
}

@InProceedings{Zhu_2023_ICCV2,
    author    = {Zhu, Kaijie and Hu, Xixu and Wang, Jindong and Xie, Xing and Yang, Ge},
    title     = {Improving Generalization of Adversarial Training via Robust Critical Fine-Tuning},
    booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
    month     = {October},
    year      = {2023},
    pages     = {4424-4434}
}

@article{wu2021attacking,
  title={Attacking adversarial attacks as a defense},
  author={Wu, Boxi and Pan, Heng and Shen, Li and Gu, Jindong and Zhao, Shuai and Li, Zhifeng and Cai, Deng and He, Xiaofei and Liu, Wei},
  journal={arXiv preprint arXiv:2106.04938},
  year={2021}
}

@inproceedings{mao2021adversarial,
  title={Adversarial attacks are reversible with natural supervision},
  author={Mao, Chengzhi and Chiquier, Mia and Wang, Hao and Yang, Junfeng and Vondrick, Carl},
  booktitle={ICCV},
  pages={661--671},
  year={2021}
}

@inproceedings{hwang2022aid,
  title={Aid-purifier: A light auxiliary network for boosting adversarial defense},
  author={Hwang, Duhun and Lee, Eunjung and Rhee, Wonjong},
  booktitle={ICPR},
  pages={2401--2407},
  year={2022},
  organization={IEEE}
}

@inproceedings{songpixeldefend,
  title={PixelDefend: Leveraging Generative Models to Understand and Defend against Adversarial Examples},
  author={Song, Yang and Kim, Taesup and Nowozin, Sebastian and Ermon, Stefano and Kushman, Nate},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{borkar2020defending,
  title={Defending against universal attacks through selective feature regeneration},
  author={Borkar, Tejas and Heide, Felix and Karam, Lina},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={709--719},
  year={2020}
}

@inproceedings{jia2019comdefend,
  title={Comdefend: An efficient image compression model to defend adversarial examples},
  author={Jia, Xiaojun and Wei, Xingxing and Cao, Xiaochun and Foroosh, Hassan},
  booktitle={CVPR},
  pages={6084--6092},
  year={2019}
}

@inproceedings{samangoueidefense,
  title={Defense-GAN: Protecting Classifiers Against Adversarial Attacks Using Generative Models},
  author={Samangouei, Pouya and Kabkab, Maya and Chellappa, Rama},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{yoon2021adversarial,
  title={Adversarial purification with score-based generative models},
  author={Yoon, Jongmin and Hwang, Sung Ju and Lee, Juho},
  booktitle={ICML},
  pages={12062--12072},
  year={2021},
  organization={PMLR}
}

@inproceedings{nie2022diffusion,
  title={Diffusion Models for Adversarial Purification},
  author={Nie, Weili and Guo, Brandon and Huang, Yujia and Xiao, Chaowei and Vahdat, Arash and Anandkumar, Animashree},
  booktitle={ICML},
  pages={16805--16827},
  year={2022},
  organization={PMLR}
}

@inproceedings{shionline,
  title={Online Adversarial Purification based on Self-supervised Learning},
  author={Shi, Changhao and Holtz, Chester and Mishne, Gal},
  booktitle={ICLR},
  year={2020}
}



@inproceedings{hillstochastic,
  title={Stochastic Security: Adversarial Defense Using Long-Run Dynamics of Energy-Based Models},
  author={Hill, Mitch and Mitchell, Jonathan Craig and Zhu, Song-Chun},
  booktitle={ICLR},
  year={2021}
}

@article{nandy2021adversarially,
  title={Adversarially Trained Models with Test-Time Covariate Shift Adaptation},
  author={Nandy, Jay and Saha, Sudipan and Hsu, Wynne and Li Lee, Mong and Zhu, Xiao Xiang},
  journal={arXiv e-prints},
  pages={arXiv--2102},
  year={2021}
}

@inproceedings{rusu2022hindering,
  title={Hindering Adversarial Attacks with Implicit Neural Representations},
  author={Rusu, Andrei A and Calian, Dan Andrei and Gowal, Sven and Hadsell, Raia},
  booktitle={ICML},
  pages={18910--18934},
  year={2022},
  organization={PMLR}
}

@inproceedings{perez2021enhancing,
  title={Enhancing adversarial robustness via test-time transformation ensembling},
  author={P{\'e}rez, Juan C and Alfarra, Motasem and Jeanneret, Guillaume and Rueda, Laura and Thabet, Ali and Ghanem, Bernard and Arbel{\'a}ez, Pablo},
  booktitle={ICCV},
  pages={81--91},
  year={2021}
}

@inproceedings{nayak2022dad,
  title={Dad: Data-free adversarial defense at test time},
  author={Nayak, Gaurav Kumar and Rawal, Ruchit and Chakraborty, Anirban},
  booktitle={WACV},
  pages={3562--3571},
  year={2022}
}

@inproceedings{hodisco,
  title={DISCO: Adversarial Defense with Local Implicit Functions},
  author={Ho, Chih-Hui and Vasconcelos, Nuno},
  booktitle={NeurIPS},
  year={2022}
}

@inproceedings{bai2019hilbert,
  title={Hilbert-based generative defense for adversarial examples},
  author={Bai, Yang and Feng, Yan and Wang, Yisen and Dai, Tao and Xia, Shu-Tao and Jiang, Yong},
  booktitle={ICCV},
  pages={4784--4793},
  year={2019}
}

@inproceedings{jin2019ape,
  title={Ape-gan: Adversarial perturbation elimination with gan},
  author={Jin, Guoqing and Shen, Shiwei and Zhang, Dongming and Dai, Feng and Zhang, Yongdong},
  booktitle={ICASSP},
  pages={3842--3846},
  year={2019},
  organization={IEEE}
}

% detection
@article{xu2017feature,
  title={Feature squeezing: Detecting adversarial examples in deep neural networks},
  author={Xu, Weilin and Evans, David and Qi, Yanjun},
  journal={arXiv preprint arXiv:1704.01155},
  year={2017}
}

@inproceedings{chen2020stateful,
  title={Stateful detection of black-box adversarial attacks},
  author={Chen, Steven and Carlini, Nicholas and Wagner, David},
  booktitle={Proceedings of the 1st ACM Workshop on Security and Privacy on Artificial Intelligence},
  pages={30--39},
  year={2020}
}

@inproceedings{li2022blacklight,
  title={Blacklight: Scalable Defense for Neural Networks against $\{$Query-Based$\}$$\{$Black-Box$\}$ Attacks},
  author={Li, Huiying and Shan, Shawn and Wenger, Emily and Zhang, Jiayun and Zheng, Haitao and Zhao, Ben Y},
  booktitle={31st USENIX Security Symposium (USENIX Security 22)},
  pages={2117--2134},
  year={2022}
}

@inproceedings{pang2020advmind,
  title={Advmind: Inferring adversary intent of black-box attacks},
  author={Pang, Ren and Zhang, Xinyang and Ji, Shouling and Luo, Xiapu and Wang, Ting},
  booktitle={Proceedings of the 26th ACM SIGKDD International Conference on Knowledge Discovery \& Data Mining},
  pages={1899--1907},
  year={2020}
}

@inproceedings{macharacterizing,
  title={Characterizing Adversarial Subspaces Using Local Intrinsic Dimensionality},
  author={Ma, Xingjun and Li, Bo and Wang, Yisen and Erfani, Sarah M and Wijewickrema, Sudanthi and Schoenebeck, Grant and Song, Dawn and Houle, Michael E and Bailey, James},
  booktitle={ICLR},
  year={2018}
}

@article{tsai2023test,
  title={Test-time Defense against Adversarial Attacks: Detection and Reconstruction of Adversarial Examples via Masked Autoencoder},
  author={Tsai, Yun-Yun and Chao, Ju-Chin and Wen, Albert and Yang, Zhaoyuan and Mao, Chengzhi and Shah, Tapan and Yang, Junfeng},
  journal={arXiv preprint arXiv:2303.12848},
  year={2023}
}

@inproceedings{moayeri2021sample,
  title={Sample efficient detection and classification of adversarial attacks via self-supervised embeddings},
  author={Moayeri, Mazda and Feizi, Soheil},
  booktitle={ICCV},
  pages={7677--7686},
  year={2021}
}

@article{papernot2018deep,
  title={Deep k-nearest neighbors: Towards confident, interpretable and robust deep learning},
  author={Papernot, Nicolas and McDaniel, Patrick},
  journal={arXiv preprint arXiv:1803.04765},
  year={2018}
}

@article{hu2019new,
  title={A new defense against adversarial images: Turning a weakness into a strength},
  author={Hu, Shengyuan and Yu, Tao and Guo, Chuan and Chao, Wei-Lun and Weinberger, Kilian Q},
  journal={NeurIPS},
  volume={32},
  year={2019}
}

@inproceedings{juuti2019prada,
  title={PRADA: protecting against DNN model stealing attacks},
  author={Juuti, Mika and Szyller, Sebastian and Marchal, Samuel and Asokan, N},
  booktitle={2019 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={512--527},
  year={2019},
  organization={IEEE}
}

@article{pang2018towards,
  title={Towards robust detection of adversarial examples},
  author={Pang, Tianyu and Du, Chao and Dong, Yinpeng and Zhu, Jun},
  journal={NeurIPS},
  volume={31},
  year={2018}
}

@article{grosse2017statistical,
  title={On the (statistical) detection of adversarial examples},
  author={Grosse, Kathrin and Manoharan, Praveen and Papernot, Nicolas and Backes, Michael and McDaniel, Patrick},
  journal={arXiv preprint arXiv:1702.06280},
  year={2017}
}

@inproceedings{metzendetecting,
  title={On Detecting Adversarial Perturbations},
  author={Metzen, Jan Hendrik and Genewein, Tim and Fischer, Volker and Bischoff, Bastian},
  booktitle={ICLR},
  year={2017}
}

@inproceedings{lu2017safetynet,
  title={Safetynet: Detecting and rejecting adversarial examples robustly},
  author={Lu, Jiajun and Issaranon, Theerasit and Forsyth, David},
  booktitle={ICCV},
  pages={446--454},
  year={2017}
}

@inproceedings{abusnaina2021adversarial,
  title={Adversarial example detection using latent neighborhood graph},
  author={Abusnaina, Ahmed and Wu, Yuhang and Arora, Sunpreet and Wang, Yizhen and Wang, Fei and Yang, Hao and Mohaisen, David},
  booktitle={ICCV},
  pages={7687--7696},
  year={2021}
}

@inproceedings{cohen2020detecting,
  title={Detecting adversarial samples using influence functions and nearest neighbors},
  author={Cohen, Gilad and Sapiro, Guillermo and Giryes, Raja},
  booktitle={CVPR},
  pages={14453--14462},
  year={2020}
}

@inproceedings{tramer2022detecting,
  title={Detecting adversarial examples is (nearly) as hard as classifying them},
  author={Tramer, Florian},
  booktitle={ICML},
  pages={21692--21702},
  year={2022},
  organization={PMLR}
}

@inproceedings{gao2021maximum,
  title={Maximum mean discrepancy test is aware of adversarial attacks},
  author={Gao, Ruize and Liu, Feng and Zhang, Jingfeng and Han, Bo and Liu, Tongliang and Niu, Gang and Sugiyama, Masashi},
  booktitle={ICML},
  pages={3564--3575},
  year={2021},
  organization={PMLR}
}

@inproceedings{deng2021libre,
  title={Libre: A practical bayesian approach to adversarial detection},
  author={Deng, Zhijie and Yang, Xiao and Xu, Shizhen and Su, Hang and Zhu, Jun},
  booktitle={CVPR},
  pages={972--982},
  year={2021}
}

@inproceedings{yang2020ml,
  title={Ml-loo: Detecting adversarial examples with feature attribution},
  author={Yang, Puyudi and Chen, Jianbo and Hsieh, Cho-Jui and Wang, Jane-Ling and Jordan, Michael},
  booktitle={AAAI},
  volume={34},
  number={04},
  pages={6639--6647},
  year={2020}
}

@inproceedings{tian2021detecting,
  title={Detecting adversarial examples from sensitivity inconsistency of spatial-transform domain},
  author={Tian, Jinyu and Zhou, Jiantao and Li, Yuanman and Duan, Jia},
  booktitle={AAAI},
  volume={35},
  number={11},
  pages={9877--9885},
  year={2021}
}

@inproceedings{bryniarskievading,
  title={Evading Adversarial Example Detection Defenses with Orthogonal Projected Gradient Descent},
  author={Bryniarski, Oliver and Hingun, Nabeel and Pachuca, Pedro and Wang, Vincent and Carlini, Nicholas},
  booktitle={ICLR}, 
  year={2022}}

@inproceedings{harder2021spectraldefense,
  title={Spectraldefense: Detecting adversarial attacks on cnns in the fourier domain},
  author={Harder, Paula and Pfreundt, Franz-Josef and Keuper, Margret and Keuper, Janis},
  booktitle={IJCNN},
  pages={1--8},
  year={2021},
  organization={IEEE}
}

@inproceedings{zhao2019adversarial,
  title={The adversarial attack and detection under the fisher information metric},
  author={Zhao, Chenxiao and Fletcher, P Thomas and Yu, Mixue and Peng, Yaxin and Zhang, Guixu and Shen, Chaomin},
  booktitle={AAAI},
  volume={33},
  number={01},
  pages={5869--5876},
  year={2019}
}

@article{feinman2017detecting,
  title={Detecting adversarial samples from artifacts},
  author={Feinman, Reuben and Curtin, Ryan R and Shintre, Saurabh and Gardner, Andrew B},
  booktitle={ICML},
  year={2017}
}

@inproceedings{li2017adversarial,
  title={Adversarial examples detection in deep networks with convolutional filter statistics},
  author={Li, Xin and Li, Fuxin},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={5764--5772},
  year={2017}
}


% Dynamic black-box defense via input/model/output perturbation
@article{qin2021random,
  title={Random noise defense against query-based black-box attacks},
  author={Qin, Zeyu and Fan, Yanbo and Zha, Hongyuan and Wu, Baoyuan},
  journal={NeurIPS},
  volume={34},
  pages={7650--7663},
  year={2021}
}

@inproceedings{xiemitigating,
  title={Mitigating Adversarial Effects Through Randomization},
  author={Xie, Cihang and Wang, Jianyu and Zhang, Zhishuai and Ren, Zhou and Yuille, Alan},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{liu2018towards,
  title={Towards robust neural networks via random self-ensemble},
  author={Liu, Xuanqing and Cheng, Minhao and Zhang, Huan and Hsieh, Cho-Jui},
  booktitle={ECCV},
  pages={369--385},
  year={2018}
}

@inproceedings{chenadversarial,
  title={Adversarial Attack on Attackers: Post-Process to Mitigate Black-Box Score-Based Query Attacks},
  author={Chen, Sizhe and Huang, Zhehao and Tao, Qinghua and Wu, Yingwen and Xie, Cihang and Huang, Xiaolin},
  booktitle={NeurIPS}, 
  year={2022}
}

@inproceedings{prakash2018deflecting,
  title={Deflecting adversarial attacks with pixel deflection},
  author={Prakash, Aaditya and Moran, Nick and Garber, Solomon and DiLillo, Antonella and Storer, James},
  booktitle={CVPR},
  pages={8571--8580},
  year={2018}
}

@inproceedings{buckman2018thermometer,
  title={Thermometer encoding: One hot way to resist adversarial examples},
  author={Buckman, Jacob and Roy, Aurko and Raffel, Colin and Goodfellow, Ian},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{he2019parametric,
  title={Parametric noise injection: Trainable randomness to improve deep neural network robustness against adversarial attack},
  author={He, Zhezhi and Rakin, Adnan Siraj and Fan, Deliang},
  booktitle={CVPR},
  pages={588--597},
  year={2019}
}

@inproceedings{lecuyer2019certified,
  title={Certified robustness to adversarial examples with differential privacy},
  author={Lecuyer, Mathias and Atlidakis, Vaggelis and Geambasu, Roxana and Hsu, Daniel and Jana, Suman},
  booktitle={2019 IEEE Symposium on Security and Privacy (SP)},
  pages={656--672},
  year={2019},
  organization={IEEE}
}

@article{wang2021fighting,
  title={Fighting gradients with gradients: Dynamic defenses against adversarial attacks},
  author={Wang, Dequan and Ju, An and Shelhamer, Evan and Wagner, David and Darrell, Trevor},
  journal={arXiv preprint arXiv:2105.08714},
  year={2021}
}

@inproceedings{chentowards,
  title={Towards Robust Neural Networks via Close-loop Control},
  author={Chen, Zhuotong and Li, Qianxiao and Zhang, Zheng},
  booktitle={ICLR},
  year={2021}
}

@article{kang2021stable,
  title={Stable neural ode with lyapunov-stable equilibrium points for defending against adversarial attacks},
  author={Kang, Qiyu and Song, Yang and Ding, Qinxu and Tay, Wee Peng},
  journal={NeurIPS},
  volume={34},
  pages={14925--14937},
  year={2021}
}

@article{gurumurthy2021joint,
  title={Joint inference and input optimization in equilibrium networks},
  author={Gurumurthy, Swaminathan and Bai, Shaojie and Manchester, Zachary and Kolter, J Zico},
  journal={NeurIPS},
  volume={34},
  pages={16818--16832},
  year={2021}
}

@article{alet2021tailoring,
  title={Tailoring: encoding inductive biases by optimizing unsupervised objectives at prediction time},
  author={Alet, Ferran and Bauza, Maria and Kawaguchi, Kenji and Kuru, Nurullah Giray and Lozano-P{\'e}rez, Tom{\'a}s and Kaelbling, Leslie},
  journal={NeurIPS},
  volume={34},
  pages={29206--29217},
  year={2021}
}

@inproceedings{chentowards,
  title={Towards Evaluating the Robustness of Neural Networks Learned by Transduction},
  author={Chen, Jiefeng and Wu, Xi and Guo, Yang and Liang, Yingyu and Jha, Somesh},
  booktitle={ICLR},
  year={2022}
}

@inproceedings{dhillonstochastic,
  title={Stochastic Activation Pruning for Robust Adversarial Defense},
  author={Dhillon, Guneet S and Azizzadenesheli, Kamyar and Lipton, Zachary C and Bernstein, Jeremy D and Kossaifi, Jean and Khanna, Aran and Anandkumar, Animashree},
  booktitle={ICLR},
  year={2018}
}

% ensemble
@inproceedings{he2017adversarial,
  title={Adversarial Example Defense: Ensembles of Weak Defenses are not Strong.},
  author={He, Warren and Wei, James and Chen, Xinyun and Carlini, Nicholas and Song, Dawn},
  booktitle={WOOT},
  pages={15--15},
  year={2017}
}

@article{abbasi2017robustness,
  title={Robustness to adversarial examples through an ensemble of specialists},
  author={Abbasi, Mahdieh and Gagn{\'e}, Christian},
  journal={arXiv preprint arXiv:1702.06856},
  year={2017}
}

@article{sengupta2017mtdeep,
  title={MTDeep: Securing deep neural nets against adversarial attacks with moving target defense},
  author={Sengupta, Sailik and Chakraborti, Tathagata and Kambhampati, Subbarao},
  booktitle="Decision and Game Theory for Security",
  year={2019}
}

@article{strauss2017ensemble,
  title={Ensemble methods as a defense to adversarial perturbations against deep neural networks},
  author={Strauss, Thilo and Hanselmann, Markus and Junginger, Andrej and Ulmer, Holger},
  journal={arXiv preprint arXiv:1709.03423},
  year={2017}
}

@inproceedings{mazeika2022steer,
  title={How to steer your adversary: Targeted and efficient model stealing defenses with gradient redirection},
  author={Mazeika, Mantas and Li, Bo and Forsyth, David},
  booktitle={ICML},
  pages={15241--15254},
  year={2022},
  organization={PMLR}
}

@inproceedings{wang2023defending,
  title={Defending black-box skeleton-based human activity classifiers},
  author={Wang, He and Diao, Yunfeng and Tan, Zichang and Guo, Guodong},
  booktitle={AAAI},
  volume={37},
  number={2},
  pages={2546--2554},
  year={2023}
}

@inproceedings{hu2019triple,
  title={Triple Wins: Boosting Accuracy, Robustness and Efficiency Together by Enabling Input-Adaptive Inference},
  author={Hu, Ting-Kuei and Chen, Tianlong and Wang, Haotao and Wang, Zhangyang},
  booktitle={ICLR},
  year={2019}
}

@inproceedings{dong2023adversarial,
  title={Adversarial Robustness via Random Projection Filters},
  author={Dong, Minjing and Xu, Chang},
  booktitle={CVPR},
  pages={4077--4086},
  year={2023}
}

@inproceedings{li2023trade,
  title={Trade-Off Between Robustness and Accuracy of Vision Transformers},
  author={Li, Yanxi and Xu, Chang},
  booktitle={CVPR},
  pages={7558--7568},
  year={2023}
}

@article{dong2022random,
  title={Random normalization aggregation for adversarial defense},
  author={Dong, Minjing and Chen, Xinghao and Wang, Yunhe and Xu, Chang},
  journal={NeurIPS},
  volume={35},
  pages={33676--33688},
  year={2022}
}

% ============================
% post-training defense






%====================================================================================================================================================================



% ====
% robust architecture & dynamic

@inproceedings{wang2019convergence,
  title={On the Convergence and Robustness of Adversarial Training},
  author={Wang, Yisen and Ma, Xingjun and Bailey, James and Yi, Jinfeng and Zhou, Bowen and Gu, Quanquan},
  booktitle={International Conference on Machine Learning},
  pages={6586--6595},
  year={2019},
  organization={PMLR}
}

@inproceedings{wu_skip_2019,
	title = {Skip Connections Matter: On the Transferability of Adversarial Examples Generated with {ResNets}},
	booktitle = {International Conference on Learning Representations},
	author = {Wu, Dongxian and Wang, Yisen and Xia, Shu-Tao and Bailey, James and Ma, Xingjun},
	year = {2019},
}

@inproceedings{huang_exploring_2021,
	title = {Exploring Architectural Ingredients of Adversarially Robust Deep Neural Networks},
	volume = {34},
	url = {https://proceedings.neurips.cc/paper_files/paper/2021/hash/2bd7f907b7f5b6bbd91822c0c7b835f6-Abstract.html},
	abstract = {Deep neural networks ({DNNs}) are known to be vulnerable to adversarial attacks. A range of defense methods have been proposed to train adversarially robust {DNNs}, among which adversarial training has demonstrated promising results. However, despite preliminary understandings developed for adversarial training, it is still not clear, from the architectural perspective, what configurations can lead to more robust {DNNs}. In this paper, we address this gap via a comprehensive investigation on the impact of network width and depth on the robustness of adversarially trained {DNNs}. Specifically, we make the following key observations: 1) more parameters (higher model capacity) does not necessarily help adversarial robustness; 2) reducing capacity at the last stage (the last group of blocks) of the network can actually improve adversarial robustness; and 3) under the same parameter budget, there exists an optimal architectural configuration for adversarial robustness. We also provide a theoretical analysis explaning why such network configuration can help robustness. These architectural insights can help design adversarially robust {DNNs}.},
	pages = {5545--5559},
	booktitle = {Advances in Neural Information Processing Systems},
	publisher = {Curran Associates, Inc.},
	author = {Huang, Hanxun and Wang, Yisen and Erfani, Sarah and Gu, Quanquan and Bailey, James and Ma, Xingjun},
	urldate = {2023-09-09},
	year = {2021},
}

@inproceedings{shao_adversarial_2022,
	title = {On the Adversarial Robustness of Vision Transformers},
	booktitle = {Annual Conference on Neural Information Processing Systems},
	author = {Shao, Rulin and Shi, Zhouxing and Yi, Jinfeng and Chen, Pin-Yu and Hsieh, Cho-jui},
	year = {2022},
}

@inproceedings{liu_exploring_2023,
	title = {Exploring the Relationship between Architectural Design and Adversarially Robust Generalization},
	pages = {4096--4107},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Liu, Aishan and Tang, Shiyu and Liang, Siyuan and Gong, Ruihao and Wu, Boxi and Liu, Xianglong and Tao, Dacheng},
	year = {2023},
}

@article{peng_robarch_2023,
	title = {{RobArch}: Designing Robust Architectures against Adversarial Attacks},
	shorttitle = {{RobArch}},
	journaltitle = {{arXiv} preprint {arXiv}:2301.03110},
	author = {Peng, {ShengYun} and Xu, Weilin and Cornelius, Cory and Li, Kevin and Duggal, Rahul and Chau, Duen Horng and Martin, Jason},
	year = {2023},
}

@article{li_importance_2023,
	title = {On the Importance of Backbone to the Adversarial Robustness of Object Detectors},
	journaltitle = {{arXiv} preprint {arXiv}:2305.17438},
	author = {Li, Xiao and Chen, Hang and Hu, Xiaolin},
	year = {2023},
}

@inproceedings{fang_patchnas_2023,
	title = {{PatchNAS}: Repairing {DNNs} in Deployment with Patched Network Architecture Search},
	volume = {37},
	shorttitle = {{PatchNAS}},
	pages = {14811--14819},
	booktitle = {Proceedings of the {AAAI} Conference on Artificial Intelligence},
	author = {Fang, Yuchu and Li, Wenzhong and Zeng, Yao and Zheng, Yang and Hu, Zheng and Lu, Sanglu},
	year = {2023},
	note = {Issue: 12},
}

@article{xiao_robustmq_2023,
	title = {{RobustMQ}: Benchmarking Robustness of Quantized Models},
	shorttitle = {{RobustMQ}},
	journaltitle = {{arXiv} preprint {arXiv}:2308.02350},
	author = {Xiao, Yisong and Liu, Aishan and Zhang, Tianyuan and Qin, Haotong and Guo, Jinyang and Liu, Xianglong},
	year = {2023},
}

@inproceedings{gu_evaluating_2022,
	title = {Evaluating model robustness to patch perturbations},
	booktitle = {{ICML} 2022 Shift Happens Workshop},
	author = {Gu, Jindong and Tresp, Volker and Qin, Yao},
	year = {2022},
}

@article{naseer_improving_2021,
	title = {On improving adversarial transferability of vision transformers},
	journaltitle = {{arXiv} preprint {arXiv}:2106.04169},
	author = {Naseer, Muzammal and Ranasinghe, Kanchana and Khan, Salman and Khan, Fahad Shahbaz and Porikli, Fatih},
	year = {2021},
}

@inproceedings{xie_intriguing_2019,
	title = {Intriguing Properties of Adversarial Training at Scale},
	booktitle = {International Conference on Learning Representations},
	author = {Xie, Cihang and Yuille, Alan},
	year = {2019},
}

@inproceedings{cazenavette_architectural_2021,
	title = {Architectural adversarial robustness: The case for deep pursuit},
	shorttitle = {Architectural adversarial robustness},
	pages = {7150--7158},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Cazenavette, George and Murdock, Calvin and Lucey, Simon},
	year = {2021},
}

@inproceedings{peng_heterogeneous_2021,
	title = {Heterogeneous Architecture Search Approach within Adversarial Dynamic Defense Framework},
	booktitle = {The {AAAI}-22 Workshop on Adversarial Machine Learning and Beyond},
	author = {Peng, Qi and Qin, Ruoxi and Liu, Wenlin and Hou, Libin and Yan, Bin and Wang, Linyuan},
	year = {2021},
}

@article{wu_wider_2021,
	title = {Do wider neural networks really help adversarial robustness?},
	volume = {34},
	pages = {7054--7067},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Wu, Boxi and Chen, Jinghui and Cai, Deng and He, Xiaofei and Gu, Quanquan},
	year = {2021},
}

@article{nakkiran_adversarial_2019,
	title = {Adversarial robustness may be at odds with simplicity},
	journaltitle = {{arXiv} preprint {arXiv}:1901.00532},
	author = {Nakkiran, Preetum},
	year = {2019},
}

@inproceedings{dai_parameterizing_2022,
	title = {Parameterizing activation functions for adversarial robustness},
	pages = {80--87},
	booktitle = {2022 {IEEE} Security and Privacy Workshops ({SPW})},
	publisher = {{IEEE}},
	author = {Dai, Sihui and Mahloujifar, Saeed and Mittal, Prateek},
	year = {2022},
}

@inproceedings{hu_triple_2019,
	title = {Triple Wins: Boosting Accuracy, Robustness and Efficiency Together by Enabling Input-Adaptive Inference},
	shorttitle = {Triple Wins},
	booktitle = {International Conference on Learning Representations},
	author = {Hu, Ting-Kuei and Chen, Tianlong and Wang, Haotao and Wang, Zhangyang},
	year = {2019},
}

@inproceedings{qendro_towards_2022,
	title = {Towards adversarial robustness with early exit ensembles},
	pages = {313--316},
	booktitle = {2022 44th Annual International Conference of the {IEEE} Engineering in Medicine \& Biology Society ({EMBC})},
	publisher = {{IEEE}},
	author = {Qendro, Lorena and Mascolo, Cecilia},
	year = {2022},
}

@article{zhou_bert_2020,
	title = {Bert loses patience: Fast and robust inference with early exit},
	volume = {33},
	shorttitle = {Bert loses patience},
	pages = {18330--18341},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Zhou, Wangchunshu and Xu, Canwen and Ge, Tao and {McAuley}, Julian and Xu, Ke and Wei, Furu},
	year = {2020},
}

@article{gao_convergence_2019,
	title = {Convergence of adversarial training in overparametrized neural networks},
	volume = {32},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Gao, Ruiqi and Cai, Tianle and Li, Haochuan and Hsieh, Cho-Jui and Wang, Liwei and Lee, Jason D.},
	year = {2019},
}

@article{tang_robustart_2021,
	title = {Robustart: Benchmarking robustness on architecture design and training techniques},
	shorttitle = {Robustart},
	journaltitle = {{arXiv} preprint {arXiv}:2109.05211},
	author = {Tang, Shiyu and Gong, Ruihao and Wang, Yan and Liu, Aishan and Wang, Jiakai and Chen, Xinyun and Yu, Fengwei and Liu, Xianglong and Song, Dawn and Yuille, Alan},
	year = {2021},
}

@inproceedings{mok_advrush_2021,
	title = {{AdvRush}: Searching for adversarially robust neural architectures},
	shorttitle = {{AdvRush}},
	pages = {12322--12332},
	booktitle = {Proceedings of the {IEEE}/{CVF} International Conference on Computer Vision},
	author = {Mok, Jisoo and Na, Byunggook and Choe, Hyeokjun and Yoon, Sungroh},
	year = {2021},
}

@article{peng_robust_2023,
	title = {Robust Principles: Architectural Design Principles for Adversarially Robust {CNNs}},
	shorttitle = {Robust Principles},
	journaltitle = {{arXiv} preprint {arXiv}:2308.16258},
	author = {Peng, {ShengYun} and Xu, Weilin and Cornelius, Cory and Hull, Matthew and Li, Kevin and Duggal, Rahul and Phute, Mansi and Martin, Jason and Chau, Duen Horng},
	year = {2023},
}

@article{dong_adversarially_2020,
	title = {Adversarially robust neural architectures},
	journaltitle = {{arXiv} preprint {arXiv}:2009.00902},
	author = {Dong, Minjing and Li, Yanxi and Wang, Yunhe and Xu, Chang},
	year = {2020},
}

@article{zhu_robust_2023,
	title = {Robust Neural Architecture Search},
	journaltitle = {{arXiv} preprint {arXiv}:2304.02845},
	author = {Zhu, Xunyu and Li, Jian and Liu, Yong and Wang, Weiping},
	year = {2023},
}

@inproceedings{hosseini_dsrna_2021,
	title = {Dsrna: Differentiable search of robust neural architectures},
	shorttitle = {Dsrna},
	pages = {6196--6205},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Hosseini, Ramtin and Yang, Xingyi and Xie, Pengtao},
	year = {2021},
}

@article{nath_rnas-cl_2023,
	title = {{RNAS}-{CL}: Robust Neural Architecture Search by Cross-Layer Knowledge Distillation},
	shorttitle = {{RNAS}-{CL}},
	journaltitle = {{arXiv} preprint {arXiv}:2301.08092},
	author = {Nath, Utkarsh and Wang, Yancheng and Yang, Yingzhen},
	year = {2023},
}

@article{ha_generalizable_2023,
	title = {Generalizable Lightweight Proxy for Robust {NAS} against Diverse Perturbations},
	journaltitle = {{arXiv} preprint {arXiv}:2306.05031},
	author = {Ha, Hyeonjeong and Kim, Minseon and Hwang, Sung Ju},
	year = {2023},
}

@inproceedings{li_trade-off_2023,
	title = {Trade-Off Between Robustness and Accuracy of Vision Transformers},
	pages = {7558--7568},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Li, Yanxi and Xu, Chang},
	year = {2023},
}

@inproceedings{yue_effective_2022,
	title = {Effective, efficient and robust neural architecture search},
	pages = {1--8},
	booktitle = {2022 International Joint Conference on Neural Networks ({IJCNN})},
	publisher = {{IEEE}},
	author = {Yue, Zhixiong and Lin, Baijiong and Zhang, Yu and Liang, Christy},
	year = {2022},
}

@inproceedings{cheng_neural_2023,
	title = {Neural Architecture Search for Wide Spectrum Adversarial Robustness},
	volume = {37},
	pages = {442--451},
	booktitle = {Proceedings of the {AAAI} Conference on Artificial Intelligence},
	author = {Cheng, Zhi and Li, Yanxi and Dong, Minjing and Su, Xiu and You, Shan and Xu, Chang},
	year = {2023},
	note = {Issue: 1},
}

@inproceedings{xie_adversarially_2023,
	title = {Adversarially Robust Neural Architecture Search for Graph Neural Networks},
	pages = {8143--8152},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Xie, Beini and Chang, Heng and Zhang, Ziwei and Wang, Xin and Wang, Daixin and Zhang, Zhiqiang and Ying, Rex and Zhu, Wenwu},
	year = {2023},
}

@inproceedings{du_learning_2021,
	title = {Learning diverse-structured networks for adversarial robustness},
	pages = {2880--2891},
	booktitle = {International Conference on Machine Learning},
	publisher = {{PMLR}},
	author = {Du, Xuefeng and Zhang, Jingfeng and Han, Bo and Liu, Tongliang and Rong, Yu and Niu, Gang and Huang, Junzhou and Sugiyama, Masashi},
	year = {2021},
}

@article{dong_random_2022,
	title = {Random normalization aggregation for adversarial defense},
	volume = {35},
	pages = {33676--33688},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Dong, Minjing and Chen, Xinghao and Wang, Yunhe and Xu, Chang},
	year = {2022},
}

@inproceedings{guo_when_2020,
	title = {When nas meets robustness: In search of robust architectures against adversarial attacks},
	shorttitle = {When nas meets robustness},
	pages = {631--640},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Guo, Minghao and Yang, Yuzhe and Xu, Rui and Liu, Ziwei and Lin, Dahua},
	year = {2020},
}

@article{xie_smooth_2020,
	title = {Smooth adversarial training},
	journaltitle = {{arXiv} preprint {arXiv}:2006.14536},
	author = {Xie, Cihang and Tan, Mingxing and Gong, Boqing and Yuille, Alan and Le, Quoc V.},
	year = {2020},
}

@article{bai_are_2021,
	title = {Are transformers more robust than cnns?},
	volume = {34},
	pages = {26831--26843},
	journaltitle = {Advances in neural information processing systems},
	author = {Bai, Yutong and Mei, Jieru and Yuille, Alan L. and Xie, Cihang},
	year = {2021},
}

@inproceedings{chen_anti-bandit_2020,
	title = {Anti-bandit neural architecture search for model defense},
	pages = {70--85},
	booktitle = {Computer Vision–{ECCV} 2020: 16th European Conference, Glasgow, {UK}, August 23–28, 2020, Proceedings, Part {XIII} 16},
	publisher = {Springer},
	author = {Chen, Hanlin and Zhang, Baochang and Xue, Song and Gong, Xuan and Liu, Hong and Ji, Rongrong and Doermann, David},
	year = {2020},
}

@inproceedings{huang_revisiting_2023,
	title = {Revisiting Residual Networks for Adversarial Robustness},
	pages = {8202--8211},
	booktitle = {Proceedings of the {IEEE}/{CVF} Conference on Computer Vision and Pattern Recognition},
	author = {Huang, Shihua and Lu, Zhichao and Deb, Kalyanmoy and Boddeti, Vishnu Naresh},
	year = {2023},
}

@article{singh_revisiting_2023,
	title = {Revisiting Adversarial Training for {ImageNet}: Architectures, Training and Generalization across Threat Models},
	shorttitle = {Revisiting Adversarial Training for {ImageNet}},
	journaltitle = {{arXiv} preprint {arXiv}:2303.01870},
	author = {Singh, Naman D. and Croce, Francesco and Hein, Matthias},
	year = {2023},
}

@article{qin_random_2021,
	title = {Random noise defense against query-based black-box attacks},
	volume = {34},
	pages = {7650--7663},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Qin, Zeyu and Fan, Yanbo and Zha, Hongyuan and Wu, Baoyuan},
	year = {2021},
}

@inproceedings{xie_mitigating_2018,
	title = {Mitigating Adversarial Effects Through Randomization},
	booktitle = {International Conference on Learning Representations},
	author = {Xie, Cihang and Wang, Jianyu and Zhang, Zhishuai and Ren, Zhou and Yuille, Alan},
	year = {2018},
}

@article{chen_adversarial_2022,
	title = {Adversarial attack on attackers: Post-process to mitigate black-box score-based query attacks},
	volume = {35},
	shorttitle = {Adversarial attack on attackers},
	pages = {14929--14943},
	journaltitle = {Advances in Neural Information Processing Systems},
	author = {Chen, Sizhe and Huang, Zhehao and Tao, Qinghua and Wu, Yingwen and Xie, Cihang and Huang, Xiaolin},
	year = {2022},
}

@inproceedings{byun_effectiveness_2022,
	title = {On the effectiveness of small input noise for defending against query-based black-box attacks},
	pages = {3051--3060},
	booktitle = {Proceedings of the {IEEE}/{CVF} Winter Conference on Applications of Computer Vision},
	author = {Byun, Junyoung and Go, Hyojun and Kim, Changick},
	year = {2022},
}


%inference backdoor detectin
@inproceedings{orion,
  author       = {Huayang Huang and
                  Qian Wang and
                  Xueluan Gong and
                  Tao Wang},
  title        = {Orion: Online Backdoor Sample Detection via Evolution Deviance},
  booktitle    = {Proceedings of the Thirty-Second International Joint Conference on
                  Artificial Intelligence, {IJCAI}},
  pages        = {864--874},
  publisher    = {ijcai.org},
  year         = {2023}
}

@inproceedings{guo2023scale,
  title={SCALE-UP: An Efficient Black-box Input-level Backdoor Detection via Analyzing Scaled Prediction Consistency},
  author={Guo, Junfeng and Li, Yiming and Chen, Xun and Guo, Hanqing and Sun, Lichao and Liu, Cong},
  booktitle={The Eleventh International Conference on Learning Representations},
  year={2023}
}

@article{nab,
  title={Backdoor Defense with Non-Adversarial Backdoor},
  author={Liu, Min and Sangiovanni-Vincentelli, Alberto and Yue, Xiangyu},
  journal={arXiv preprint arXiv:2307.15539},
  year={2023}
}

@inproceedings{liu2023detecting,
  title={Detecting Backdoors During the Inference Stage Based on Corruption Robustness Consistency},
  author={Liu, Xiaogeng and Li, Minghui and Wang, Haoyu and Hu, Shengshan and Ye, Dengpan and Jin, Hai and Wu, Libing and Xiao, Chaowei},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={16363--16372},
  year={2023}
}

@inproceedings{freak,
  title={Don't FREAK Out: A Frequency-Inspired Approach to Detecting Backdoor Poisoned Samples in DNNs},
  author={Al Kader Hammoud, Hasan Abed and Bibi, Adel and Torr, Philip HS and Ghanem, Bernard},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2337--2344},
  year={2023}
}

@inproceedings{simclr,
  title={A simple framework for contrastive learning of visual representations},
  author={Chen, Ting and Kornblith, Simon and Norouzi, Mohammad and Hinton, Geoffrey},
  booktitle={International conference on machine learning},
  pages={1597--1607},
  year={2020},
  organization={PMLR}
}

@inproceedings{byun2022effectiveness,
  title={On the effectiveness of small input noise for defending against query-based black-box attacks},
  author={Byun, Junyoung and Go, Hyojun and Kim, Changick},
  booktitle={Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision},
  pages={3051--3060},
  year={2022}
}

@inproceedings{aithal2022boundary,
  title={Boundary Defense Against Black-box Adversarial Attacks},
  author={Aithal, Manjushree B and Li, Xiaohua},
  booktitle={2022 26th International Conference on Pattern Recognition (ICPR)},
  pages={2349--2356},
  year={2022},
  organization={IEEE}
}

% discussion---------------------------start
@inproceedings{sun2021can,
  title={Can shape structure features improve model robustness under diverse adversarial settings?},
  author={Sun, Mingjie and Li, Zichao and Xiao, Chaowei and Qiu, Haonan and Kailkhura, Bhavya and Liu, Mingyan and Li, Bo},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={7526--7535},
  year={2021}
}

@inproceedings{wang2021backdoorl,
  title={BACKDOORL: Backdoor Attack against Competitive Reinforcement Learning},
  author={Wang, Lun and Javed, Zaynah and Wu, Xian and Guo, Wenbo and Xing, Xinyu and Song, Dawn},
  booktitle={30th International Joint Conference on Artificial Intelligence, IJCAI 2021},
  pages={3699--3705},
  year={2021},
  organization={International Joint Conferences on Artificial Intelligence}
}

@inproceedings{guan2023attacking,
  title={Attacking Neural Networks with Neural Networks: Towards Deep Synchronization for Backdoor Attacks},
  author={Guan, Zihan and Sun, Lichao and Du, Mengnan and Liu, Ninghao},
  booktitle={Proceedings of the 32nd ACM International Conference on Information and Knowledge Management},
  pages={608--618},
  year={2023}
}

@inproceedings{qi2022revisiting,
  title={Revisiting the assumption of latent separability for backdoor defenses},
  author={Qi, Xiangyu and Xie, Tinghao and Li, Yiming and Mahloujifar, Saeed and Mittal, Prateek},
  booktitle={The eleventh international conference on learning representations},
  year={2022}
}

%% certified backdoor defense zml

@article{wang2020certifying,
  title={On certifying robustness against backdoor attacks via randomized smoothing},
  author={Wang, Binghui and Cao, Xiaoyu and Gong, Neil Zhenqiang and others},
  journal={arXiv preprint arXiv:2002.11750},
  year={2020}
}

@inproceedings{rosenfeld2020certified,
  title={Certified robustness to label-flipping attacks via randomized smoothing},
  author={Rosenfeld, Elan and Winston, Ezra and Ravikumar, Pradeep and Kolter, Zico},
  booktitle={International Conference on Machine Learning},
  pages={8230--8241},
  year={2020},
  organization={PMLR}
}

@inproceedings{weber2023rab,
  title={Rab: Provable robustness against backdoor attacks},
  author={Weber, Maurice and Xu, Xiaojun and Karla{\v{s}}, Bojan and Zhang, Ce and Li, Bo},
  booktitle={2023 IEEE Symposium on Security and Privacy (SP)},
  pages={1311--1328},
  year={2023},
  organization={IEEE}
}


% jia2021intrinsic

@inproceedings{levine2021deep,
  title={Deep Partition Aggregation: Provable Defense against General Poisoning Attacks},
  author={Levine, A and Feizi, S},
  booktitle={International Conference on Learning Representations (ICLR)},
  year={2021}
}

% jia2022certified


@inproceedings{ji2022crab,
  title={CRAB: Certified Patch Robustness Against Poisoning-Based Backdoor Attacks},
  author={Ji, Huxiao and Li, Jie and Wu, Chentao},
  booktitle={2022 IEEE International Conference on Image Processing (ICIP)},
  pages={2486--2490},
  year={2022},
  organization={IEEE}
}

% zhang2022bagflip

@inproceedings{pham2022verifying,
  title={Verifying Neural Networks Against Backdoor Attacks},
  author={Pham, Long H and Sun, Jun},
  booktitle={International Conference on Computer Aided Verification},
  pages={171--192},
  year={2022},
  organization={Springer}
}
@inproceedings{cohen2019certified,
  title={Certified adversarial robustness via randomized smoothing},
  author={Cohen, Jeremy and Rosenfeld, Elan and Kolter, Zico},
  booktitle={international conference on machine learning},
  pages={1310--1320},
  year={2019},
  organization={PMLR}
}
%%
% certified adversarial defense

@inproceedings{li2023sok,
  title={Sok: Certified robustness for deep neural networks},
  author={Li, Linyi and Xie, Tao and Li, Bo},
  booktitle={2023 IEEE symposium on security and privacy (SP)},
  pages={1289--1310},
  year={2023},
  organization={IEEE}
}

@inproceedings{katz2017reluplex,
  title={Reluplex: An efficient SMT solver for verifying deep neural networks},
  author={Katz, Guy and Barrett, Clark and Dill, David L and Julian, Kyle and Kochenderfer, Mykel J},
  booktitle={Computer Aided Verification: 29th International Conference, CAV 2017, Heidelberg, Germany, July 24-28, 2017, Proceedings, Part I 30},
  pages={97--117},
  year={2017},
  organization={Springer}
}

@inproceedings{gehr2018ai2,
  title={AI2: Safety and robustness certification of neural networks with abstract interpretation},
  author={Gehr, Timon and Mirman, Matthew and Drachsler-Cohen, Dana and Tsankov, Petar and Chaudhuri, Swarat and Vechev, Martin},
  booktitle={2018 IEEE symposium on security and privacy (SP)},
  pages={3--18},
  year={2018},
  organization={IEEE}
}

@article{singh2018fast,
  title={Fast and effective robustness certification},
  author={Singh, Gagandeep and Gehr, Timon and Mirman, Matthew and P{\"u}schel, Markus and Vechev, Martin},
  journal={Advances in neural information processing systems},
  volume={31},
  year={2018}
}

@inproceedings{lecuyer2019certified,
  title={Certified robustness to adversarial examples with differential privacy},
  author={Lecuyer, Mathias and Atlidakis, Vaggelis and Geambasu, Roxana and Hsu, Daniel and Jana, Suman},
  booktitle={2019 IEEE symposium on security and privacy (SP)},
  pages={656--672},
  year={2019},
  organization={IEEE}
}

% cohen2019certified  

% discussion---------------------------end








==> sections/section-deployment.tex <==
\subsection{Deployment-stage Defense against weight attack}
\label{sec: defense at deployment}


While the adversarial weight attack occurs at the deployment stage, there are also a few defenses adopted at the same stage to mitigate the weight attack effect. 
For example, the output code matching (OCM) method \cite{ozdenizci2022improving} proposed to replace the usual one-hot encoding of classes by partially overlapping bit strings, through changing the softmax layer to a N-length output layer with tanh activation function, such that the bits of representing different classes are correlated.
Consequently, the cost to achieve a successful weight attack to a particular target class will be increased, and the benign accuracy of other classes will be significantly influenced. 
%
The Aegis method \cite{wang2023aegis} observed that existing targeted weight attacks often flipped some critical bits in higher layers (\ie., layers close to the output). Inspired by this observation, Aegis adopted a dynamic-exit mechanism to attach extra internal classifiers (ICs) to hidden layers, such that the inference of each input sample could early-exit from different intermediate layers, to mitigate the weight attack effect in higher layers. 
%
The randomized rotated and nonlinear encoding (RREC) method \cite{liu2023generating} adopted two strategies to enhance the tolerance to bit flips in weight attack, including 1) randomized rotation to obfuscate the bit order of weights, to reduce the chance of identifying vulnerable bits, and 2) nonlinear quantization function of weights to reduce the bit-flip distance. 
%
The DeepAttest method \cite{chen2019deepattest} firstly designed a device-specific fingerprint, and encoded it into the model weights deployed on the device, while storing it in a trusted execution environment (TEE) of the same device. Then, at the inference stage, the fingerprint was extracted from the model. If the extracted fingerprint is consistent with that stored in TEE, then the model was verified and could be used for inference. 

In addition to the above defense methods designed for adversarial weight attacks (\ie, targeted), there are also several weight manipulation detection methods for any weight manipulation attacks, including both targeted and untargeted weight attacks. We refer readers to \cite{qian2023survey} for more details about these detection-based defense methods.  





==> sections/section-discussion-backup.tex <==
\newpage
\section{Discussions}
\label{sec: discussion}
In this section, we discuss 
We turn to discussing some further research issues which have recently drawn much attentions in robust adversarial training, hoping to oﬀer more inspirations and outlooks in this ﬁeld. We will review from three aspects: Interpretability of adversarial examples, robust generalization, and robustness evaluation.

\paragraph{Is it possible to design a defense to improve the robustness against different attack paradigms simultaneously?} If possible, is there any feasible solution? Although there are a few works focuse on improving robustness in multi-perspective, we believe that composite defense at different stages is a solution for improving the robustness against different attack paradigms simultaneously. Previous works \cite{weng2020trade,zhao2020bridging,sun2021can} have analyzed the relationship between adversarial robustness and backdoor robustness. Weng \etal \cite{weng2020trade} raised that the robustness of a DNN against adversarial attacks contradicts its robustness against backdoor attacks by empirical study. They also point that this trade-off is not entirely detrimental to existing defenses and a model unlearns backdoors after adversarial training in some cases \cite{wang2019neural}.
Sun \etal \cite{sun2021can} explore model robustness under different attack scenarios and they find  that forces models to rely more on edge features can boost model robustness under adversarial attacks and backdoor attacks. Zhao \etal \cite{zhao2020bridging} utilize mode connectivity to repair backdoored models and improve adversarial resistance. To conclude, robustness against different attack paradigms can be accommodated in a model and we believe the composite defenses is a promising and important direction in the feature.

 On the other hand, adversarial robustness are commonly utilized to remove backdoors in backdoor defense works \cite{wang2019neural,zeng2022adversarial,mu2023progressive,zhu2023neural}. PBE \cite{mu2023progressive} argues that the adversarial examples computed by backdoor models and the poisoned samples show similarity in the feature space. Therefore, enhancing adversarial robustness can deactivate poisoned samples in the backdoored model. Nevertheless, a more comprehensive examination of the intricate relationship between these factors remains an unresolved issue and the pursuit of a robust model that combines both adversarial robustness and backdoor robustness continues to be a valuable avenue for research. 
% 在某一个阶段、针对某一种攻击的防御，对于其他攻击有什么影响
% discussion肯定要分析不同类型/阶段的防御的差异
% \paragraph{One-stage vs multi-stage defenses(horizontally)}
% Apart from defenses in individual stage, there are also plenty of works that operate in multi-stages where it's assumed that defenders can acquire and revise models in several stages. It is common in backdoor defenses. 

% \paragraph{vertical: adversarial vs backdoor}
% 加个 discuss 说二者的联系吧 利用对抗做后门的，研究后门的对抗性质种种
\paragraph{Challenges \& oppotunity}
Despite the impressive huge growth of defense works, defenses against AML are still in their infancy. The shortcomings and worries can be summarized as follows:
\begin{itemize}
    \item Defending against the attack-agnostic scenario: In real-world applications, attackers may employ a wide range of strategies, from subtle perturbations on queried data to implanting backdoors into the model. As attackers continually develop new and sophisticated methods, defense strategies designed for specific attack types may become less effective. Attack-agnostic defenses need to be applicable in real-world, dynamic environments, where they need to account for this diversity and remain effective in the face of evolving adversarial techniques. Addressing these concerns requires a shift towards more adaptive and robust defense strategies. And it is valuable to provide a resilient foundation for machine learning systems in the face of an ever-changing threat landscape.
    \item Defending against the domain-agnostic scenario: A critical concern lies in the scarcity of approaches tailored for domain-agnostic scenarios. The worry arises from the diverse characteristics and data distributions inherent in different domains such as CV, NLP, audio, and multi-modal models. Current defense strategies, often designed for specific domains, may struggle to generalize effectively, leaving certain applications vulnerable to adversarial exploits. To address this gap, future work should prioritize the development of defenses capable of seamlessly adapting across various application areas, ensuring resilience against adversarial threats regardless of the specific domain.
    \item Defense method based on weaker assumptions: Specifically, there is a growing worry about the limited availability of defenses that operate under less restrictive conditions, such as data-free, black-box, and model-structure-agnostic scenarios. The current landscape of defenses often relies on strong assumptions about data availability, model architectures, or white-box access, rendering them less practical in real-world, dynamic settings. The future imperative lies in developing defenses that can operate effectively without access to extensive training data, in scenarios where the internal workings of the model are not fully known, and across diverse model structures. Exploring defense methods based on weaker assumptions is pivotal for enhancing the applicability and robustness of defense mechanisms in the face of evolving and sophisticated adversarial threats, paving the way for more resilient machine learning systems in practical, less controlled environments.
    \item Defense against training paradigms-agnostic scenarios: Another concern is defenses across different paradigms, particularly in the context of the prevailing importance of semi-supervised and self-supervised learning. As these alternative paradigms, exemplified by their prominent role in the development of foundation models, gain prominence, the current dearth of defenses tailored to safeguard them against adversarial threats becomes more pronounced. By extending the focus beyond traditional supervised learning, researchers can explore more dimensions of defense strategies that align with emerging paradigms, ensuring a more comprehensive and versatile defense against adversarial threats in evolving and dynamic learning environments.
    \item Developing more comprehensive evaluation metrics: A critical concern is the deficiency of comprehensive evaluation metrics. The prevailing focus on attack success rates and model accuracy metrics overlooks essential aspects, particularly the temporal and computational costs associated with defense mechanisms, which are also crucial for real-world applications. Future research should prioritize the development of nuanced metrics that encompass both computational dimensions and defending effects against different aspects of attacks, offering a more encompassing evaluation of defense strategies. 
\end{itemize}

\textbf{1) Backdoor defense}: Although numerous backdoor defense works have considerable performance based on different phenomena, such as quick learning of backdoors \cite{li2021anti}, transformation-robustness difference between poisoned samples and clean samples \cite{chen2022effective,guo2023scale}, parameters-perturbation sensitivity \cite{anp,zheng2022data}, it still remains challenging to clearly explain why these phenomena exist on backdoor learning tasks and their intricate interconnections. As the field of backdoor attack methods advances, it becomes increasingly apparent that existing defense mechanisms can invariably be circumvented. Consequently, the persistence of the backdoor threat stands as a critical and pressing subject demanding comprehensive investigation, such as the intricate characteristic of backdoored models, their landscape, \etc

\textbf{2) Adversarial defense}: 
\ding{182} \emph{It is hard to find the optimal solution.} In adversarial defense, identifying the optimal solution remains a challenging task. A notable demonstration of this challenge is the persistent presence of adversarial examples within models. This difficulty in achieving optimality may stem from the inherently complex nature of the solution space or finding the optimum within the constraints of finite data/searching steps. Despite continuous efforts in defense strategies, the existence of adversarial examples underscores the need for future research to delve deeper into refining optimization approaches or exploring novel methodologies that can address the inherent challenges in achieving an optimal defense solution,  both theoretically and empirically.
\ding{183} \textit{Poor performance on both adversarial training and certified defense methods}. The observed poor performance in both adversarial training, the mainstream approaches in adversarial defense, and certified defense methods highlights a significant trade-off between robustness and accuracy. While AT aims to enhance robustness, it often comes at the expense of accuracy, and certified defense methods, theoretically reliable, struggle to reconcile both aspects effectively in many cases. This inherent trade-off poses a considerable challenge in striking a balance between model resilience to adversarial attacks and maintaining high accuracy in practical applications. Future research should focus on innovatively addressing this trade-off, offering a more practical solution in real-world machine learning scenarios. \ding{184} \textit{Robustness gap between adversarial robustness with human perception.} The substantial disparity between adversarial robustness and the robustness perceived by the human eye presents a formidable challenge in the field of adversarial defense. For example, adversarial robustness is typically constrained within a 0.3 \(l_p\)-norm bound, whereas human perception remains robust within even a 30 \(l_p\)-norm bound. This significant difference in robustness thresholds poses a considerable hurdle for existing adversarial defense mechanisms. Future research should focus on understanding the nuanced perceptual robustness of human vision and leveraging this insight to develop defense strategies that bridge the gap between model robustness and human visual tolerance. 

\textbf{3) Weight defense}: As for weight defense, three pivotal aspects demand attention for future research: interpretability, the synergy between adversarial training and weight defense, and the combination of weight perturbation and pruning strategies.  \ding{182} \textit{Interpretability of existing methods}: A critical problem for advancing weight defense lies in enhancing the interpretability of current methods. Understanding how weight adjustments impact model behavior is crucial for refining defense mechanisms. Future research should delve into developing transparent frameworks that illuminate the intricate relationships between weight modifications and model robustness. This interpretability not only aids in refining existing methods but also instills confidence in the deployment of weight defense strategies. \ding{183} \textit{Differences and combinations between AT and weight defense}: The intersection of adversarial training and weight defense is a potential approach. While AT fortifies models against input perturbations, weight defense mechanisms contribute to robustness with weight perturbation resilience. Investigating their symbiotic relationship and potential combination could yield a comprehensive defense strategy that is robust against a wider array of adversarial challenges.
\ding{184} \textit{Combination of Perturbation and Pruning}: The combination between weight perturbation and weight pruning presents an intriguing avenue for future research. Combining the perturbation strategy's simplicity and efficiency with model pruning could yield a more potent defense mechanism. Researchers should explore innovative ways to harmonize these techniques that optimally balances robustness and model performance.

\paragraph{Defense in other fields}
% reinforce learning/unsupervised Learning/NLP/3D point/video/multi-mode

\begin{itemize}
    \item Backdoor: Apart from supervised learning paradiam in image classification tasks, backdoor defenses have gained prominence in various fields of machine learning, including unsupervised Learning, reinforce learning, natural language processing, 3D point colud, video analysis, and multi-modal learning. In \textbf{unsupervised Learning}, it aims to discover patterns and structures in data without labels. Some recent works \red{cite} have demonstrated the susceptibility of DNNs to unsupervised learning. Followed by these threat, backdoor defenses in unsupervised learning also propose robust training strategies \red{cite} to cut off the relationship between triggers and target labels, such as disentangled representation \red{cite}. In \textbf{reinforcement learning} \red{cite}, agents learn to interact with an environment to maximize a cumulative reward. Backdoor attacks can occur when an adversary introduces subtle biases in the environment and provides incorrect rewards for specific behaviors, confusing the agent within their designed environment \red{cite}. The main challenge in backdoor defenses is the dynamic and adaptive nature of RL environments. RL environments can be highly complex and dynamic, making it challenging to detect subtle biases or vulnerabilities that can be exploited by attackers. Detecting when the reward signal is being tampered with and distinguishing it from legitimate changes in the environment is also a non-trivial task. RLBackdoor \cite{wang2021backdoorl} uses game-theoretical approaches and adversarial training to detect and mitigate backdoor attacks. In \textbf{natural language processing}(NLP), backdoor attacks can involve manipulating text data to induce unintended behaviors in NLP models, such as bias or toxic responses. The main challenge in NLP backdoor defense is identifying and mitigating subtle linguistic manipulations introduced by attackers. Defenses in these filed is like that in image classifications, \ie, identifying poisoned training data and designing models robust to adversarial inputs \red{cite}. 
    There are also some works in \textbf{3D Point Cloud Data}, \textbf{video analysis}, and \textbf{multi-modal learning}, \textbf{foundation models} \red{cite}. These works considers more realistic csenarios in real-world and challenges specific to each domain, showing the growing concern of backdoor attacks across various machine learning paradiams. 
    \item Adversarial defense: \red{TODO} \textcolor{red}{RL, Unsupervised, Few-shot, MoE}
    \item weight defense: \red{TODO}
\end{itemize}

\paragraph{Theories}
As discussed previously, the majority of existing works are confined to empirical evaluations of defense performance, and they cannot ensure robustness against unknown attacks. Consequently, these defenses may be susceptible to adaptive attacks from sophisticated adversaries \red{cite:adaptive attack}. In addressing this issue, alternative approaches known as certified defense methods have been proposed. These methods, under certain assumptions, offer reliable and certified robustness against any form of attack.

\textbf{1) Backdoor defense:} Existing empirical backdoor defenses are proposed based on the characteristic of existing attacks, and their effectiveness is sensitive in real applications. Moreover, they have no theoretical guarantees on their performance against different attacks and new stronger of adaptive attacks are constantly proposed \cite{guan2023attacking,qi2022revisiting}. To prevent such a cat-and-mouse game, Wang \etal \cite{wang2020certifying} takes the first step towards certified defenses against backdoor attacks via the randomized smoothing technique, which was originally proposed to certify robustness against adversarial examples \cite{cohen2019certified}. In \cite{wang2020certifying}, the smoothed function is built based on a base function which takes data vector as an input and outputs a label, and the smoothed function adds random noise to the input data vector to make the base function a provably robust one. Then a certified radius could be computed as a guarantee to avoid attacks. A similar instantiation of randomized smoothing is used in \cite{rosenfeld2020certified} to defend against label-flipping attacks and their variant obtains the certified bounds with minimal additional runtime complexity compared to standard classification. 
Moreover, CRAB \cite{ji2022crab} is another certified defense against patched backdoor attacks, and it proposes two 
different randomized smoothing method depending on fixed-region or randomized-region triggers. BagFlip \cite{zhang2022bagflip} is another randomized smoothing approach that combines bagging of the training set and noising of the training data and the test input by randomly flipping features and labels. Model ensemble technique is also utilized in some works \cite{jia2021intrinsic,levine2021deep,jia2022certified} to obtain certified robustness against backdoor attacks. More recently, RAB \cite{weber2023rab} provides a unified framework via randomized smoothing techniques on model robustness, and proposes the first robust training process to smooth the trained model.
A crucial limitation of existing certified defenses against backdoor attacks is that they only guarantee $l_p$-norm bounded perturbations of triggers. However, this assumption may not always be valid in real-world applications where the trigger can be unbounded and inconspicuous. Therefore, there is a need for a sophisticated certified defense approach for backdoor learning that goes beyond the framework of adversarial learning, which remains under-explored.

\textbf{2) Adversarial defense:} 
Certified robustness is a rapidly developed approach within adversarial defense, and there are also some surveys available \red{cite} in this area. Certiﬁed robustness is typically categorized into two main branches: \textit{robustness verification} \red{cite} and \textit{robust training} \red{cite}. The former seeks to evaluate a model's robustness by establishing a theoretically certified lower bound of robustness under specific perturbation constraints (\eg, $l_{\infty}$-norm bounded perturbation). The latter involves training models with the objective of achieving high certified robustness. 
Existing \textit{robustness verification} approaches can be classified into two categories: deterministic verification and probabilistic verification \cite{li2023sok}. In cases where the provided input is non-robust against an attack, deterministic verification ensures an output of "not verified". For example, Reluplex \cite{katz2017reluplex} is an early work towards certified robustness of networks that provides a formulation for satisfiability modulo theories (SMT) solver for the DNNs with ReLUs. Later works \cite{gehr2018ai2,singh2018fast} focus on building deterministic verification robustness on more complex networks. In these works, a proven lower bound is usually provided to establish the minimal perturbation necessary to alter a model's decision.
On the other hand, probabilistic verification guarantees an output of "not verified" with a specified probability, where the randomness is independent of the input. This kind of approaches first establishes a smoothed classifier by adding random noises into a function and then a certiﬁed robustness is derived on this smoothed classifier. PixelDP \cite{lecuyer2019certified} and \cite{cohen2019certified} are two classical works that build smoothed classifier by differential privacy and Neyman Pearson lemma, respectively. 
Among \textit{robustness verification} approaches, the main challenge is that they either demand extensive computations to rigorously certify the robustness of the model, especially for large and complex models, or they output trivial bounds that are overly simplistic and do not adequately capture the nuanced behavior of the model \cite{li2023sok}. To improve model robustness, \textit{robust training} approaches are proposed which making modiﬁcations to the learning algorithm. \textit{Robust training} approaches can be roughly divided into \textit{Regularization-based methods} \red{cite}, which focus on avoiding changes in the decision boundaries by small variation on the input of the algorithm by regularization on Lipschitz constant or expanding the decision boundaries, \textit{Relaxation-based methods} \red{cite}, which use the computed bounds from linear relaxation as the training objective to explicitly improve robustness, and \textit{Augmentation based method} \red{cite}, which trains the model with noisy inputs by Data augmentation.

\textbf{3) Weight defense:} So far as we know, certified robustness against weight attacks is underexplored, and there is no work on this topic. One reason could be that it is too hard to guarantee robustness against the weight change for such a complex nonlinear DNN.

% theoretical robustness bounds which do not generalize to different attacks and threat models studied. A promising research path is the investigation of properties that can theoretically guarantee general lower bounds of robustness to adversarial attacks

\paragraph{Applications}
Although defense methods are primarily designed for protecting neural networks from different types of attacks, these methods can be used beyond the scope of model robustness, and have some other applications. In this section, we briefly introduce some recent works for the application of defense methods.
\begin{itemize}
    \item \textbf{Adversarial Training for Improving OOD Generalization} Out-of-distribution (OOD) data are data that do not follow the same distribution as the training data, and may cause the neural network to produce inconsistent and incomprehensible predictions. Improving the OOD generalization of neural networks is a challenging and important problem, especially in safety-critical and security-sensitive domains. Some works have pointed out the connection between input-robustness and OOD generalization, and show that adversarial training can improve the OOD generalization of neural networks \cite{yi2021improved, xin2023connection}. For example, \textcolor{red}{some work} 

    \item \textbf{Weight Defense} \textcolor{red}{TODO} 
    
    \item \textbf{Backdoor Defense for Evaluating Copying Protection} Recent works have explored the use of backdoor attacks for ownership verification and copy protection for pre-trained models and datasets. The idea is to embed a backdoor watermark into the model or the data, and use it to prove the ownership or the authenticity of the model or the data. For example, \textcolor{red}{Some Works}

    To evaluate the backdoor-based methods, backdoor detection and backdoor defense methods can serve as evaluation methods. These methods aim to determine whether the model or the data is poisoned by a backdoor attack, and identify or remove the backdoor watermark.  For example, \textcolor{red}{Some Works} 
\end{itemize}



% bess. One typical application ackd'bu's'toor defense: evaluate IP
% Adversarial Training: 
% 

% \paragraph{Emerging trends}


